Connectivity in Random Annulus Graphs and the Geometric Block Model

We provide new connectivity results for {\em vertex-random graphs} or {\em random annulus graphs} which are significant generalizations of random geometric graphs. Random geometric graphs (RGG) are one of the most basic models of random graphs for spatial networks proposed by Gilbert in 1961, shortly after the introduction of the Erd\H{o}s-R\'{en}yi random graphs. They resemble social networks in many ways (e.g. by spontaneously creating cluster of nodes with high modularity). The connectivity properties of RGG have been studied since its introduction, and analyzing them has been significantly harder than their Erd\H{o}s-R\'{en}yi counterparts due to correlated edge formation. Our next contribution is in using the connectivity of random annulus graphs to provide necessary and sufficient conditions for efficient recovery of communities for {\em the geometric block model} (GBM). The GBM is a probabilistic model for community detection defined over an RGG in a similar spirit as the popular {\em stochastic block model}, which is defined over an Erd\H{o}s-R\'{en}yi random graph. The geometric block model inherits the transitivity properties of RGGs and thus models communities better than a stochastic block model. However, analyzing them requires fresh perspectives as all prior tools fail due to correlation in edge formation. We provide a simple and efficient algorithm that can recover communities in GBM exactly with high probability in the regime of connectivity.

==> soda.tex <==
%%\def\year{2018}\relax
%%File: formatting-instruction.tex
%\documentclass[letter,11pt]{article} %DO NOT CHANGE THIS
%\usepackage[
%  margin=3cm,
%  includefoot,
%  footskip=30pt,
%]{geometry}
%%\usepackage{times}  %Required
%\usepackage{url,hyperref}  %Required
%\usepackage{graphicx}  %Required
%%\usepackage[round]{natbib}
%\usepackage[round]{natbib}
%%\frenchspacing  %Required
%%\setlength{\pdfpagewidth}{8.5in}  %Required
%%\setlength{\pdfpageheight}{11in} 
%
%%\usepackage{nips_2017}
%
%% to compile a camera-ready version, add the [final] option, e.g.:
%% \usepackage[final]{nips_2017}
%\setcounter{secnumdepth}{2} 
%%\usepackage[utf8]{inputenc} % allow utf-8 input
%%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%%\usepackage{hyperref}       % hyperlinks
%\usepackage{times}
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{amsthm}
%\usepackage{algorithm}
%\usepackage{bbold}
%\usepackage{tikz}
%\usetikzlibrary{decorations.pathreplacing}
%\usetikzlibrary{patterns}
%\usepackage{amsmath}
%\usepackage{algorithmic}
%\usepackage{verbatim}
%\usepackage{subcaption}
%%\usepackage{cite}
%\usepackage{graphicx}
%\usepackage{multirow}
%\usepackage{amssymb}
%\usepackage{color}
%\usepackage{caption}
%%\usepackage{subfig}
%\usepackage{enumitem}
%\usepackage{hyphenat}
%\usepackage{array}
%\usepackage{booktabs}
%\usepackage{wrapfig}
%\usepackage{relsize}
%\usepackage{tikz}
%%\usepackage{subfig}
%
%\usepackage{afterpage}
%\usetikzlibrary{arrows}
%\title{Connectivity in Random Annulus Graphs and the Geometric Block Model}
%
%\author{
%Sainyam Galhotra \quad Arya Mazumdar \quad Soumyabrata Pal \quad Barna Saha 
% \thanks{College of Information and Computer Sciences,
%  University of Massachusetts Amherst,
%  Amherst, MA 01003,
%  \texttt{\{sainyam,arya,spal,barna\}@cs.umass.edu}. This research is supported by NSF  awards  CCF 1642550, CCF 1464310 and CAREER awards  1642658 and 1652303.}
%  %% examples of more authors
%}
%\sloppy
%\DeclareGraphicsExtensions{.eps}
%
%\newcommand\nc\newcommand
%\nc\bfa{{\boldsymbol a}}\nc\bfA{{\boldsymbol A}}\nc\cA{{\mathcal A}}
%\nc\bfb{{\boldsymbol b}}\nc\bfB{{\boldsymbol B}}\nc\cB{{\mathcal B}}
%\nc\bfc{{\boldsymbol c}}\nc\bfC{{\boldsymbol C}}\nc\cC{{\mathcal C}}
%\nc\sC{{\mathscr C}}
%\nc\bfd{{\boldsymbol d}}\nc\bfD{{\boldsymbol D}}\nc\cD{{\mathcal D}}
%\nc\bfe{{\boldsymbol e}}\nc\bfE{{\boldsymbol E}}\nc\cE{{\mathcal E}}
%\nc\bff{{\boldsymbol f}}\nc\bfF{{\boldsymbol F}}\nc\cF{{\mathcal F}}
%\nc\bfg{{\boldsymbol g}}\nc\bfG{{\boldsymbol G}}\nc\cG{{\mathcal G}}
%\nc\bfh{{\boldsymbol h}}\nc\bfH{{\boldsymbol H}}\nc\cH{{\mathcal H}}
%\nc\bfi{{\boldsymbol i}}\nc\bfI{{\boldsymbol I}}\nc\cI{{\mathcal I}}
%\nc\bfj{{\boldsymbol j}}\nc\bfJ{{\boldsymbol J}}\nc\cJ{{\mathcal J}}
%\nc\bfk{{\boldsymbol k}}\nc\bfK{{\boldsymbol K}}\nc\cK{{\mathcal K}}
%\nc\bfl{{\boldsymbol l}}\nc\bfL{{\boldsymbol L}}\nc\cL{{\mathcal L}}
%\nc\bfm{{\boldsymbol m}}\nc\bfM{{\boldsymbol M}}\nc\sM{{\mathscr M}}\nc\cM{{\mathcal M}}
%\nc\bfn{{\boldsymbol n}}\nc\bfN{{\boldsymbol N}}\nc\cN{{\mathcal N}}
%\nc\bfo{{\boldsymbol o}}\nc\bfO{{\boldsymbol O}}\nc\cO{{\mathcal O}}
%\nc\bfp{{\boldsymbol p}}\nc\bfP{{\boldsymbol P}}\nc\cP{{\mathcal P}}
%\nc\bfq{{\boldsymbol q}}\nc\bfQ{{\boldsymbol Q}}\nc\cQ{{\mathcal Q}}
%\nc\bfr{{\boldsymbol r}}\nc\bfR{{\boldsymbol R}}\nc\cR{{\mathcal R}}
%\nc\bfs{{\boldsymbol s}}\nc\bfS{{\boldsymbol S}}\nc\cS{{\mathcal S}}
%\nc\bft{{\boldsymbol t}}\nc\bfT{{\boldsymbol T}}\nc\cT{{\mathcal T}}
%\nc\bfu{{\boldsymbol u}}\nc\bfU{{\boldsymbol U}}\nc\cU{{\mathcal U}}
%\nc\bfv{{\boldsymbol v}}\nc\bfV{{\boldsymbol V}}\nc\cV{{\mathcal V}}
%\nc\bfw{{\boldsymbol w}}\nc\bfW{{\boldsymbol W}}\nc\cW{{\mathcal W}}
%\nc\bfx{{\boldsymbol x}}\nc\bfX{{\boldsymbol X}}\nc\cX{{\mathcal X}}
%\nc\bfy{{\boldsymbol y}}\nc\bfY{{\boldsymbol Y}}\nc\cY{{\mathcal Y}}
%\nc\bfz{{\boldsymbol z}}\nc\bfZ{{\boldsymbol Z}}\nc\cZ{{\mathcal Z}}
%
%
%\nc\diff{{\mathrm d}}
%\nc\e{{\mathrm e}}
%\nc\calC{{\mathcal C}}
%%\ncG{{\mathcal G}}
%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
%
%\DeclareMathOperator{\supp}{supp}
%\DeclareMathOperator{\average}{avg}
%
%\DeclareMathOperator{\rank}{rank}
%\DeclareMathOperator{\Var}{var}
%\DeclareMathOperator{\Col}{col}
%\DeclareMathOperator{\wt}{wt}
%\DeclareMathOperator{\sgn}{sgn}
%
%\newcommand{\remove}[1]{}
%\newcommand{\correct}[1]{\textcolor{black}{#1}}
%\newcommand{\latest}[1]{\textcolor{red}{#1}}
%
%
%
%\newcommand{\h}{h_\mathrm{B}}
%\newcommand{\avg}{{\mathbb E}}
%\newcommand{\expect}{{\mathbb E}}
%\newcommand{\dist}{d_{L}}
%\newcommand{\rdss}{\mathbb{CAP}}
%\newcommand{\indx}{\mathrm{INDEX}}
%\newcommand{\len}{\mathrm{len}}
%\newcommand{\minrank}{\mathrm{minrank}}
%
%
%\newcommand{\eps}{\varepsilon}
%\newcommand{\tO}{{\tilde{O}}}
%
%\newtheorem*{lemma*}{Lemma}
%\newtheorem{corollary}{Corollary}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}
%\newtheorem{proposition}{Proposition}
%\theoremstyle{definition}
%\newtheorem{definition}{Definition}
%\newtheorem*{corollaryn}{Corollary}
%\newtheorem{observation}[theorem]{Observation}
%\newtheorem{problem}{Problem}
%\newtheorem{example}{Example}
%\newtheorem{remark}{Remark}
%\newtheorem{claim}{Claim}
%\newtheorem{conclusion}{Conclusion}
%
%
%%\theoremstyle{theorem-n}
%%\newtheorem*{theorem-n}{Theorem}
%%\newtheorem*{lemma-n}{lemma}
%\newcommand{\minp}{\otimes}
%
%\newcommand{\cc}{{\sf Query-Cluster}}
%
%
%\newcommand{\Ex}{{\mathbb{E}}}
%
%\setlength{\belowdisplayskip}{0pt} \setlength{\belowdisplayshortskip}{0pt}
%\setlength{\abovedisplayskip}{0pt} \setlength{\abovedisplayshortskip}{0pt}
%
%
%\def\DEBUG{true}
%
%\ifdefined\DEBUG
%\newcommand{\barn}[1]{\textcolor{red}{#1}}
%\newcommand{\arya}[1]{\textcolor{green}{#1}}
%
%% \newcommand{\uri}[1]{\textcolor{magenta}{#1}}
%  \def\rem#1{{\marginpar{\raggedright\scriptsize #1}}}
%  \newcommand{\barnr}[1]{\rem{\textcolor{red}{$\bullet$ #1}}}
%  \newcommand{\aryar}[1]{\rem{\textcolor{green}{$\bullet$ #1}}}
%%  \newcommand{\urir}[1]{\rem{\textcolor{magenta}{$\bullet$ #1}}}
%\else
%
%  \newcommand{\arya}[1]{#1}
%  \newcommand{\barn}[1]{#1}
% 
%%  \newcommand{\uri}[1]{#1}
% 
%  \newcommand{\barnr}[1]{}
%  \newcommand{\aryar}[1]{}
%%  \newcommand{\urir}[1]{}
%
%\fi
%
%\newcommand\reals{{\mathbb R}}
%\newcommand\complexes{{\mathbb C}}
%\newcommand\ff{{\mathbb F}}
%\newcommand\bK{{\mathbb K}}
%\newcommand\integers{{\mathbb Z}}
%\newcommand\rationals{{\mathbb Q}}
%
%
%\allowdisplaybreaks
%
%
%
%
%
%\begin{document}
%% \nipsfinalcopy is no longer used
%
%\maketitle

%\begin{abstract}
%Random geometric graphs are the simplest, and perhaps the earliest possible random graph model of spatial networks, introduced by Gilbert in 1961. In the most basic setting, a random geometric graph $G(n,r)$ has  $n$ vertices. Each vertex of the graph is assigned a real number  in $[0,1]$ randomly and uniformly. There is an edge between two vertices if the corresponding two random numbers differ by at most $r$ (to mitigate the boundary effect, let us consider the Lee distance here, $d_L(u,v) = \min\{|u-v|, 1-|u-v|\}$). It is well-known that the connectivity threshold regime for  random geometric graphs is at $r \approx \frac{\log n}{n}$. In particular, if $r = \frac{a\log n}{n}$, then a random geometric graph  is connected with high probability if and only if $a > 1$. Consider $G(n,\frac{(1+\epsilon)\log{n}}{n})$ for any $\epsilon >0$ to satisfy the connectivity requirement and delete half of its edges which have distance at most $\frac{\log{n}}{2n}$. It is natural to believe that the resultant graph will be disconnected. Surprisingly, we show that the graph still remains connected! 

%Formally, generalizing random geometric graphs, we define a random annulus graph $G(n, [r_1, r_2]), r_1 <r_2$ with $n$ vertices.   Each vertex of the graph is assigned a real number  in $[0,1]$ randomly and uniformly as before. There is an edge between two vertices if the Lee distance between the corresponding two random numbers is between $r_1$ and $r_2$, $0<r_1<r_2$. Let us assume $r_1 = \frac{b \log n}{n},$ and $r_2 = \frac{a \log n}{n}, 0 <b <a$. We show that this graph is connected with high probability if and only if $a -b > \frac12$ and $a >1$. That is $G(n, [0,\frac{0.99\log n}{n}])$ is not connected but $G(n,[\frac{0.50 \log n}{n},\frac{1+\epsilon \log n}{n}])$  is.


%This result  is  then used in finding the recovery threshold of {\em geometric block model}, a random graph based model for real-world communities defined based on geometric random graphs analogous to the popular stochastic block model. Geometric block model is a basic random graph model for spatial communities, and as shown in an earlier work, is a better model than the stochastic block model for a variety of different community detection problems, especially as it captures correlated edge formulation. In a geometric block model with two equally sized communities, each community is represented by $G(n,r_s)$ whereas the inter-cluster edges are formed according to $G(n,r_d)$, $r_s > r_d$. In the regime, where $r_s,r_d = \Theta(\frac{\log n }{n})$, we study the necessary and sufficient conditions (on $r_s,r_d$) for recovery of the two parts exactly from the graph. To  show the sufficiency, we provide an efficient algorithm for recovery of the  partition,  a significant improvement on previously available results. The analysis of the algorithm crucially uses aforementioned curious threshold phenomenon of random annulus graphs. The necessary condition that we provide is also the first nontrivial lower bound on this problem. 
%\end{abstract}

%\section{Introduction-SODA}
%
%Models of random graphs are ubiquitous with Erd\H{o}s-R\'{en}yi graphs \citep{erdos1959random,gilbert1959random} at the forefront. Studies of the properties of random graphs had led to many fundamental theoretical observations as well as many engineering applications. The introduction of random geometric graphs (RGG) shortly follows that of Erd\H{o}s-R\'{en}yi graphs \citep{gilbert1961random}, and they constitute the first and simplest model of spatial networks. The one-dimensional RGG $G(n,r), n \in \mathbb{Z}_+, r \in (0,2\pi]$ is defined in the following way. It is a graph with  $n$ vertices. Each vertex $u$ is assigned a random number $X_u$ selected randomly and uniformly from $[0,2\pi]$. Two vertices $u$ and $v$ are connected by an edge, if and only if $d_L(X_u,X_v) \equiv \min\{|X_u-X_v|, 2\pi-|X_u-X_v|\} \le r.$ This model can straightforwardly be extended to higher dimensional case, where vertices are assigned random (possible non-uniform) points from some closed compact subset of the Euclidean space  and then two vertices will have an edge between them if the inner product between the corresponding vectors is higher than some prescribed value. Random geometric graphs have several desirable properties that model real human social networks, such as vertices with high modularity and the degree associativity property (high degree nodes tend to connect). This has led RGGs to be used as models of disease outbreak in social network \citep{eubank2004modelling} and flow of opinions \citep{zhang2014opinion}. RGGs are also a popular model for wireless (ad-hoc) communication networks \citep{dettmann2016random,haenggi2009stochastic}. Recent works on RGGs also include hypothesis testing between an Erd\H{o}s-R\'{en}yi graph and a random geometric graph \citep{bubecktriangle}.
%
%Threshold properties of random graphs (especially Erd\H{o}s-R\'{en}yi graphs) have been at the center of much theoretical interest, and in particular it is known  that many graph properties exhibit sharp phase transition phenomena \citep{friedgut1996every}. Random geometric graphs also exhibit similar threshold properties; in particular, the connectivity threshold for RGGs is known to be at $r =\frac{\log n}{n}$ for the one-dimensional model defined above \citep{penrose2003random}.
%
%Consider the random geometric graph $G(n,r)$ defined above with $r = \frac{a\log n}{n}$\footnote{The base of the logarithm is $e$ unless otherwise mentioned.}. The threshold property says that $G(n,r)$ is connected with high probability if and only if $a > 1$\footnote{That is, $G(n,\frac{1+\epsilon\log n}{n})$ is connected for any $\epsilon >0$. We will ignore this $\epsilon$ and just mention connectivity threshold as $\frac{\log{n}}{n}$}. Now let us consider a variant of $G(n,\frac{\log n}{n})$, where instead of two points $u,v$ having edges when $d_L(X_u,X_v)/\frac{\log n}{n} \le 1$, two points will have an edge between them if and only if $\delta \le d_L(X_u,X_v)/\frac{\log n}{n} \le 1, \delta>0$. Clearly this graph has less edges than $G(n,\frac{\log n}{n})$.  Is this graph still connected?
%Surprisingly, we show that the above modified graph remains connected as long as $\delta \le 0.5$. Note that, on the other hand,  $G(n,\frac{(1-\delta)\log n}{n})$ is not connected for any $\delta >0$. 
%
%To formalize this point, let us define a mild generalization of RGG, called the random annulus graph (RAG). Given two numbers $0 \le r_1\le r_2\le 1$, the random annulus graph ${\rm RAG}(n, [r_1,r_2])$ is a random graph with $n$ vertices. Each vertex $u$ is assigned a random number $X_u$ selected randomly and uniformly from $[0,2\pi]$. Two vertices $u$ and $v$ are connected by an edge, if and only if $r_1 \le d_L(X_u,X_v) \le r_2$. Therefore, for $r_1 =0$, random annulus graph ${\rm RAG}(n,[0,r_2])$ is simply the random geometric graph $G(n,r_2)$.  Random annulus graphs  have been previously mentioned in \citep{dettmann2016random}. The interval $[r_1,r_2]$ is called the connectivity interval in RAG.
%
%Now consider an  ${\rm RAG}(n,[r_1,r_2])$ when $r_1 = \frac{b\log n}{n}$ and $r_2 = \frac{a \log n}{n}$. We show that when $b >0$, the random annulus graph  ${\rm RAG}(n,[\frac{b\log n}{n},\frac{a\log n}{n}])$ is connected with high probability if and only if $a - b > 0.5$ and $a > 1$. This means the graphs ${\rm RAG}(n, [0, \frac{0.99 \log n}{n}])$ and ${\rm RAG}(n, [\frac{0.49 \log n}{n}, \frac{0.99 \log n}{n}])$ are not connected with high probability, whereas ${\rm RAG}(n, [\frac{0.50 \log n}{n}, \frac{\log n}{n}])$ is connected. Note that, since we are using the Lee distance (or geodesic distance), this fact cannot be intuitively justified by boundary effects. For a depiction of the connectivity regime for the random annulus graph $G(n,[\frac{b\log n}{n},\frac{a\log n}{n}])$ see Figure~\ref{fig:region}.
%
%Can we explain this seemingly curious shift in connectivity interval, when one goes from $b=0$ to $b >0$? Compare the RAG$(n, [\frac{0.50 \log n}{n}, \frac{\log n}{n}])$ with the ${\rm RAG}(n, [0, \frac{\log n}{n}])$. The former one can  be thought of being obtained by deleting all the `short-distance' edges from the later. It turns out  the `long-distance' edges are  sufficient to maintain connectivity, because they can connect points over multiple hops in the graph. This intriguing observation of  {\em long edge phenomenon} in random geometric graphs is one of the major contributions of this paper. 
%
%
%
%%We have not found similar examples in the literat 
%
%%This surprising fact does not carry over to the higher dimensions of random geometric graphs. \textcolor{red}{Write results for higher dimension here}% In stead we are able to show that the for a similar setting, the length of connectivity interval remains 
%
%We are motivated to study the threshold phenomena of random annulus graphs, because it appears naturally in the analysis of the geometric block model (GBM) \citep{galhotra2017geometric}.
%The geometric block model is a  probabilistic generative model of communities in a variety of networks and is a spatial analogue to the popular stochastic block model (SBM) \citep{holland1983stochastic,dyer1989solution,decelle2011asymptotic,abbe2015community,abh:16,DBLP:conf/colt/HajekWX15,chin2015stochastic,mossel2015consistency,agarwal2017multisection}. The SBM %is a random graph model for community detection that
% generalizes the
%Erd\H{o}s-R\'{en}yi graphs in the following way. Consider a graph $G(V,E)$, where $V = V_1 \sqcup V_2 \sqcup \dots \sqcup V_k$ is a disjoint union of $k$ clusters denoted by $V_1, \dots, V_k.$ The edges of the graph are drawn randomly: there is an edge between $u \in V_i$ and $v \in V_j$ with probability $q_{i,j}, 1\le i,j \le k.$
%Given the adjacency matrix of such a graph, the task is to find exactly (or approximately) the partition $V_1 \sqcup V_2 \sqcup \dots \sqcup V_k$ of $V$.
%
%This model has been incredibly popular both in theoretical and practical domains of community detection. Recent theoretical works  focus on characterizing sharp threshold of recovering the partition in the SBM. For example, when there are only two communities of exactly equal sizes, and the inter-cluster edge probability is $\frac{b\log n}{n}$ and intra-cluster edge probability is $\frac{a\log n}{n}$, it is known that exact recovery is possible if and only if $\sqrt{a} - \sqrt{b} > \sqrt{2}$ 
%\citep{abh:16,mossel2015consistency}. The regime of the probabilities being $\Theta\Big(\frac{\log n}{n}\Big)$ has been put forward as one of most interesting ones, because  in an Erd\H{o}s-R\'{en}yi random graph, this is the threshold for graph connectivity \citep{bollobas1998random}. %This result has been subsequently generalized for $k$ communities \cite{abbe2015community,abbe2015recovering,hajek2016achieving} (for constant $k$ or when $k=o(\log{n})$), and under the assumption that the communities are generated according to a probabilistic generative model (there is a prior probability $p_i$ of an element being in the $i$th community) \cite{abbe2015community}. 
%Note that the results are not only of theoretical interest, many real-world networks exhibit a ``sparsely connected'' community feature \citep{leskovec2008statistical}, and any efficient recovery algorithm for sparse SBM has many potential applications.  
%
%While SBM is a popular model (because of its apparent simplicity), there are many aspects of real social networks, such as  ``transitivity rule'' (`friends having common friends') inherent to many social and other community structures, are not accounted for in SBM.  
%To circumvent this, in a previous work, we proposed a random graph community detection model analogous to the stochastic block model, that we call the {\em geometric block model} (GBM) \citep{galhotra2017geometric}. The GBM depends on the basic definition of the random geometric graph in  the same way the SBM depends on  Erd\H{o}s-R\'{en}yi graphs. The two-cluster GBM with vertex set $V= V_1\sqcup V_2$, $V_1 = V_2$ is a random graph defined in the following way. Suppose, $0 \le r_d < r_s \le 1$ be two  real numbers. For each vertex $u \in V$ randomly and independently choose a number $X_u \in [0,2\pi]$ according to uniform distribution. There will be an edge between $u,v$ if and only if,
%\begin{align*}
%d_L(X_u, X_v) \le r_s & \text{ when } u, v \in V_1 \text{ or } u,v \in V_2\\
% d_L(X_u, X_v) \le r_d & \text{ when } u \in V_1, v \in V_2 \text{ or } u\in V_2,v \in V_1.
%\end{align*}
%Let us denote this random graph as ${\rm GBM}(r_s,r_d)$. Given this graph  ${\rm GBM}(r_s,r_d)$, the main problem of community detection is to find the parts $V_1$ and $V_2$.
%
%
%% To be precise, consider any three vertices $x, y$ and $z$. If $x$ and $y$ are connected by an edge (or they are in the same community), and $y$ and $z$ are connected by an edge (or they are in the same community), then it is more likely than not that $x$ and $z$ are connected by an edge. This phenomenon can be seen in many network structures - predominantly in social networks, blog-networks and advertising. SBM, primarily a generalization of Erd\"{o}s-Renyi random graph, does not take into account this characteristic, and in particular, probability of an edge between $x$ and $z$ there is independence of the fact that there exist edges between $x$ and $y$ and $y$ and $z$. However, one needs to be careful such that by allowing such ``transitivity'', the simplicity and elegance of the SBM is not lost.
%
%%Inspired by the above question The GBM depends on the basic definition of the {\em random geometric graph}. % that has found a lot of practical use in wireless networking because of its inclusion of the notion of proximity between nodes \cite{penrose2003random}.
%
%It has been shown in  \citep{galhotra2017geometric} that GBM accurately represents (more so than SBM) many real world networks such as Amazon product metadata or DBLP citation and collaboration networks. A simple motif-counting algorithm was also provided in   \citep{galhotra2017geometric}, that provably works well in the sparse regime of $r_s, r_d \sim \frac{\log n}{n}$ and real sparse networks. In contrast, the simple motif counting can easily seen to perform badly in SBM, giving some further validation of GBM in real networks, where such algorithms are often very effective.
%
%Motivated by SBM literature, we here also look at GBM in the connectivity regime, i.e., when $r_s = \frac{a\log n}{n}, r_d = \frac{b\log n}{n}.$ Our first contribution in this part is to provide a lower bound that shows that it is impossible to recover the parts from ${\rm GBM}(\frac{a\log n}{n},\frac{b\log n}{n})$ when 
%$
%a - b < 1/2.
%$
%We also provide a simple, intuitive, and efficient triangle-counting algorithm that  leads to significant improvement over the algorithm proposed in  \citep{galhotra2017geometric}. 
%The algorithm simply count the number of common neighbors for each pair in the GBM connected by an edge, and deletes some edges when the number of common neighbors is below some threshold. In the next step of the algorithm we just find connected components in the redacted graph.
%The relation between $a$ and $b$ that defines a sufficient condition of recovery in ${\rm GBM}(\frac{a\log n}{n},\frac{b\log n}{n})$ has been derived as one of the main results of this paper (see, Theorem~\ref{gbm:upper}). 
%
%%The recovery region is plotted  in Figure \textcolor{red}{Here}
%
%To analyze the algorithm proposed, we need to  crucially use the results obtained for the connectivity of random annulus graphs. Indeed, we need to go beyond the scenario for RAG when the connectivity interval can be disjoint, such as ${\rm RAG}(n, [0,r_1]\cup[r_2,r_3])$ where $0 <r_1<r_2 <r_3\le 1$. 
%
%It is possible to generalize the GBM to include different distributions, different metric spaces, multiple parts and higher dimensions. It is also possible to construct other type of spatial block models such as the one very recently being put forward in \citep{sankararaman2018community} which rely on the random dot product graphs \citep{young2007random}. In \citep{sankararaman2018community}, edges are drawn between vertices randomly and independently as a function  of the distance between the corresponding vertex random variables. In contrast, in GBM edges are drawn deterministically given the vertex random variables, and edges are dependent unconditionally. \citep{sankararaman2018community} also considers the recovery scenario where in addition to the graph, values of the vertex random variables are provided. In GBM, we only observe the graph. In particular, it will be later clear from our derivations that if we are given the corresponding random variables (locations) to the variables in addition to the graph, then recovery of the partitions in ${\rm GBM}(\frac{a\log n}{n},\frac{b\log n}{n})$ is possible if and only if $a - b > 0.5, a>1$.
%
%The paper is organized as follows. In Section \ref{sec:notation}, we provide the main results of the paper formally. In Section~\ref{sec:rag}, the sharp connectivity phase transition results for random annulus graphs are proven. In Section~\ref{sec:gbm}, a lower bound for the geometric block model as well as the main recovery algorithm and its analysis are presented.
%

\section{1-D Random Annulus Graphs: Proof of Theorem \ref{thm:rag}}
\label{sec:rag}

In this section we prove Theorem~\ref{thm:rag}. Towards this proof we show the sufficient condition first and delegate the necessary condition at the end of this section.

First, we show that the area of region $B(u,r)=\{ x \mid  x \in S^t, x \le r\}$ is proportional to $r^t$. It is one of the key lemmas that will be helpful  throughout the proof.
\begin{lemma}
The area of the region $B(u,r)=\{ x \mid  x \in S^t, d(u,x) \le r\}$ is $c_tr^t$ for $r=o(1)$ where $c_t \approx \frac{\pi^{t/2}}{\Gamma (\frac{t}{2}+1) }$\label{lem:area}
\end{lemma}
\begin{proof}
We use the following fact from \cite{larsen2017improved} for the proof. For a sphere of radius $1$, the hyperspherical cap of angular radius $\theta= \max_{x \in B(u,r)} \arccos \langle x,u \rangle$ has a surface area $C_t(\theta)$ given by 
\begin{align*}
C_t(\theta)=\int_{0}^{\tan \theta} \frac{S_{t-1}(r)}{(1+r^{2})^{2}}dr 
\end{align*}
where $S_{t-1}(\theta)=\frac{t\pi^{t/2}}{\Gamma (\frac{t}{2}+1) }\theta^{t-1}$. From the definition of $B(u,r)$ we have that $\cos \theta=1-\frac{r^{2}}{2}$ and therefore $\tan \theta=\frac{r \sqrt{4-r^{2}}}{2-r^{2}} \approx r$. Now since $r=o(1)$ and $1+r^{2}$ is an increasing function of $r$, we must have that 
\begin{align*}
\int_{0}^{r} \frac{t\pi^{t/2}}{(1+o(1))\Gamma (\frac{t}{2}+1) }\theta^{t-1} d\theta  < C_t(\theta) <  \int_{0}^{r} \frac{t\pi^{t/2}}{\Gamma (\frac{t}{2}+1) }\theta^{t-1} d\theta
\end{align*}
and therefore $C_t(\theta)$ can be expressed as $c_t r^t$ where $c_t$ lies in $\Big(\frac{\pi^{t/2}}{(1+o(1))\Gamma (\frac{t}{2}+1) },\frac{\pi^{t/2}}{\Gamma (\frac{t}{2}+1) } \Big)$
\end{proof}

\begin{corollary}
For $t=1$, the area of the region $B(u,r)=\{ x \mid  x \in S^t, d(u,x) \le r\}$ is $cr$ for $r=o(1)$ where $c \approx \frac{\pi^{1/2}}{\Gamma (\frac{3}{2}) }=2$\label{lem:1dArea}
\end{corollary}
We use this Lemma to calculate the length of the arc around $u$  within a distance $r$ and other probability calculations.
%lower bound (impossibility result) first.

\subsection{Sufficient condition for connectivity of RAG}


%Next, we show the sufficient condition for connectivity for random annulus graphs. 
\begin{theorem}\label{thm:upper}
The random annulus graph ${\rm RAG}(n,[\frac{b\log n}{n},\frac{a\log n}{n}])$  is connected with  probability $1-o(1)$ if $a >2\pi$ and $a - b >\pi $.
\end{theorem}
To prove this theorem we use two main technical lemmas that show two different events happen with high probability simultaneously. 

\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-20pt}
\centering
\begin{tikzpicture}[thick, scale=0.5]
 \filldraw[color=black, fill=red!0,  line width=2pt](0,0) circle (3.5);
 \draw [line width=2pt, color=black!60,->](0,0) -- (3.5,0)node[anchor=north east] at (2,0) {$1$};
 \filldraw [gray] (0,0) circle (2pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
\filldraw [red] (0,3.5) circle (2pt);% node[anchor=north east] at (0,3.9){u};
\filldraw [red] (3.5,0) circle (2pt);% node[anchor=north east] at (0,3.9){u};
\filldraw [red] (0,-3.5) circle (2pt);% node[anchor=north east] at (0,3.9){u};
\filldraw [red] (-3.5,0) circle (2pt);% node[anchor=north east] at (0,3.9){u}
\filldraw [red] (2.47,2.47) circle (2pt);% node[anchor=north east] at (0,3.9){u};
\filldraw [red] (2.47,-2.47) circle (2pt);% node[anchor=north east] at (0,3.9){u};
\filldraw [red] (-2.47,2.47) circle (2pt);% node[anchor=north east] at (0,3.9){u};
\filldraw [red] (-2.47,-2.47) circle (2pt);% node[anchor=north east] at (0,3.9){u};;
\draw[red]    (0,3.5) to[out=80,in=40] (2.47,2.47);
\draw[red]    (2.47,2.47) to[out=40,in=60](3.5,0) ;
\draw[red]    (3.5,0) to[out=40,in=-50](2.47,-2.47) ;
\draw[red]    (2.47,-2.47) to[out=-20,in=-60](0,-3.5) ;
\draw [red]   (0,-3.5) to[out=-100,in=-100](-2.47,-2.47) ;
\draw [red]   (-2.47,-2.47) to[out=-120,in=-200](-3.5,0) ;
\draw [red]   (-3.5,0) to[out=150,in=-180](-2.47,2.47) ;
\draw [red]   (-2.47,2.47) to[out=150,in=100](0,3.5) ;
\filldraw [blue] (3.23,1.339) circle (2pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
\filldraw [blue] (3.23,-1.339) circle (2pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
\filldraw [blue] (-3.23,1.339) circle (2pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
\filldraw [blue] (-3.23,-1.339) circle (2pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
\filldraw [blue] (1.339,3.23) circle (2pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
\filldraw [blue] (1.339,-3.23) circle (2pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
\filldraw [blue] (-1.339,3.23) circle (2pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
\filldraw [blue] (-1.339,-3.23) circle (2pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
\draw[blue]   (3.23,1.339) to[out=10,in=10, , distance=2cm](3.23,-1.339);
\draw[blue]    (3.23,-1.339) to[out=-20,in=-60, distance=2cm](1.339,-3.23) ;
\draw[blue]    (1.339,-3.23) to[out=-80,in=-80,distance=2cm](-1.339,-3.23) ;
\draw[blue]    (-1.339,-3.23) to[out=-100,in=-150,distance=2cm](-3.23,-1.339) ;
\draw[blue]    (-3.23,-1.339) to[out=-150,in=150,distance=2cm](-3.23,1.339) ;
\draw[blue]    (-3.23,1.339) to[out=120,in=150,distance=2cm](-1.339,3.23) ;
\draw[blue]    (-1.339,3.23) to[out=120,in=50,distance=2cm](1.339,3.23) ;
\draw[blue]    (1.339,3.23) to[out=20,in=50,distance=2cm](3.23,1.339) ;
\end{tikzpicture}
\caption{Each vertex having two neighbors on either direction implies the graph is a union of cycles. The cycles can be interleaving in $[0,2\pi]$.\label{fig:arr0}}
\end{wrapfigure}



\begin{lemma}\label{lem:lemma1}
A set of vertices $\cC \subseteq V$ is called a cover of $[0,2\pi]$, if for any point $y$ in $[0,2\pi]$ there exists a vertex $v\in \cC$ such that $d(v,y) \le \frac{a\log n}{2n}$.  A ${\rm RAG}(n, [\frac{b\log n}{n}, \frac{a\log n}{n}])$ is a union of cycles  %$\{\cC =(w_1\to w_2\to \dots\to w_\ell\to w_1)\}$ 
such that every cycle forms a cover of $[0,2\pi]$  (see Figure~\ref{fig:arr0}) as long as $a-b >\pi$ and $a >2\pi$ with  probability $1-o(1)$.
\end{lemma}
We consider this lemma to be a main technical contribution for this paper and a large part of this section is dedicated to the proof. 
This lemma also shows effectively the fact that `long-edges' are able to connect vertices over multiple hops.
%(\textcolor{red}{Mention long edge phenomena}).
Note that, the statement of Lemma~\ref{lem:lemma1} would be easier to prove if the condition were $a-b>2\pi$. 
In that case what we prove is that every vertex  has neighbors (in the RAG) on both of the left and right directions. To  see this
%In order to prove the above statement, we  define  two events that together imply connectivity   and then show that the events simultaneously occur with high probability. 
 %The first event is that 
for each vertex $u$ , assign two indicator $\{0,1\}$-random variables $A_{u}^{l}$ and $A_{u}^{r}$, with $A_{u}^{l}=1$ if and only if there is no node $x$ to the left of node $u$ such that $d(u,x) \in [\frac{b\log n}{n},\frac{a\log n}{n}]$. Similarly, let $A_{u}^{r}=1$ if and only if there is no node $x$ to the right of node $u$ such that $d(u,x)\in [\frac{b\log n}{n},\frac{a\log n}{n}]$. Now define $A=\sum_{u}( A_{u}^{l}+A_{u}^{r})$.  We have, 
$$\Pr(A_{u}^{l})=\Pr(A_{u}^{r})=(1-\frac{(a-b)\log n}{2\pi n})^{n-1},$$ 
and, 
$$\avg[A]=2n(1-\frac{(a-b)\log n}{2\pi n})^{n-1} \le 2n^{1-\frac{(a-b)}{2\pi}}.$$
 If $a-b >2\pi$ then $\avg[A]=o(1)$ which implies, by invoking Markov inequality, that with high probability every node will have neighbors (connected by an edge in the RAG) on either side. This results in the interesting conclusion that every vertex will lie in  cycle that covers  $[0,2\pi]$. This is true for every vertex, hence the graph is simply a union of cycles each of which is a cover of $[0,2\pi]$.
The main technical challenge is to show that this conclusion remains valid even when $a-b >\pi$, which is proved after we describe the other components of the result in this section. %at the end of this section.

\begin{lemma}\label{lem:lemma2}
Set two real numbers $k\equiv \lceil b/(a-b)\rceil+1$ and $\epsilon < \frac \pi {2k}$. In an ${\rm RAG}(n, [\frac{b\log n}{n}, \frac{a\log n}{n}]), 0 <b <a$, with  probability $1-o(1)$ there exists a vertex $u_0$ and  $k$ nodes $\{u_1, u_2 ,\ldots, u_k\}$ to the right of $u_0$ such that $d(u_0,u_i) \in [\frac{(i(a-b)-2i\epsilon)\log n}{n},\frac{(i(a-b)-(2i-1)\epsilon) \log n}{n}]$ and  $k$ nodes $\{v_1, v_2 ,\ldots, v_k\}$ to the right of $u_0$ such that $d(u_0,v_i) \in [\frac{((i(a-b)+b-(2i-1)\epsilon)\log n}{n},\frac{(i(a-b)+b -(2i-2)\epsilon)\log n}{n}]$, for $i =1,2,\ldots,k$. The arrangement of the vertices is shown  in Figure~\ref{fig:arr}.
\end{lemma}

With  the help of these two lemmas, we are in a position to  prove Theorem~\ref{thm:upper}. The proof of  the two lemmas are given immediately after the proof of the theorem.

\begin{proof}[Proof of Theorem~\ref{thm:upper}]
We have shown that the two events mentioned in Lemmas \ref{lem:lemma1} and \ref{lem:lemma2} happen with high probability. Therefore they simultaneously happen under the condition $a>2\pi$ and $a-b >\pi$.
%\begin{itemize}
%\item  every vertex will lie in a cycle $(w_1\to w_2\to \dots\to w_\ell)$ with locations on the vertices appearing in the increasing order in  $[0,1]$;
%\item  there exists a node $u_0$ and exactly $k\equiv \lceil b/(a-b)\rceil+1$ nodes $\{u_1, u_2 ,\ldots, u_k\}$ to the right of $u_0$ such that $d(u_0,u_i) \in [\frac{(i(a-b)-2i\epsilon)\log n}{n},\frac{(i(a-b)-(2i-1)\epsilon) \log n}{n}]$ and exactly $k$ nodes $\{v_1, v_2 ,\ldots, v_k\}$ to the right of $u_0$ such that $d(u_0,v_i) \in [\frac{((i(a-b)+b-(2i-1)\epsilon)\log n}{n},\frac{(i(a-b)+b -(2i-2)\epsilon)\log n}{n}]$, for $i =1,2,\ldots,k$.
%\end{itemize}
Now we will show that these events together imply that the graph is connected. To see this, consider the vertices $u_0,\{u_1, u_2, \ldots, u_k\}$ and $\{v_1, v_2, \ldots, v_k\}$ that satisfy the conditions of Lemma \ref{lem:lemma2}. We can observe that each vertex $v_i$ has an edge with $u_i$ and $u_{i-1}$, $i =1, \ldots,k$. This is because (see Figure~\ref{fig:arr} for a depiction)
$$
d(u_i,v_i) %&\ge d(v_i,u_0) - d(u_i,u_0)\\
 \ge \frac{((i(a-b)+b-(2i-1)\epsilon)\log n}{n} - \frac{i(a-b)-(2i-1)\epsilon) \log n}{n}= \frac{b \log n}{n} \quad \text{and}
$$ 
\begin{align*}
 d(u_i,v_i) &\le %|\max(d(v_i,u_0)) - \min(d(u_i,u_0)) |\\
   \frac{i(a-b)+b -(2i-2)\epsilon\log n}{n} - \frac{(i(a-b)-2i\epsilon)\log n}{n} = \frac{(b + 2\epsilon)\log n}{n}.
\end{align*}

Similarly, 
\vspace{-10pt}
\begin{align*}
d(u_{i-1},v_i)& %\ge |\min(d(v_i,u_0)) - \max(d(u_{i-1},u_0))| \\
\ge \frac{((i(a-b)+b-(2i-1)\epsilon)\log n}{n} - \frac{(i-1)(a-b)-(2i-3)\epsilon) \log n}{n}\\
& = \frac{(a-2\epsilon)\log n}{n} \quad \text{and}
\end{align*}
\begin{align*}
d(u_{i-1},v_i) %& \le |\max(d(v_i,u_0)) - \min(d(u_{i-1},u_0))| \\
&\le \frac{i(a-b)+b -(2i-2)\epsilon\log n}{n} - \frac{((i-1)(a-b)-2(i-1)\epsilon)\log n}{n} = \frac{a\log n}{n}.
\end{align*}
 This implies that $u_0$ is connected to $u_i$ and $v_i$ for all $i=1,\dots,k$. The first event implies that %all vertices have neighbors on either side and therefore the 
 the connected components are cycles spanning the entire line $[0,2\pi]$.
 Now consider two such disconnected components, one of which consists of the nodes $u_0,\{u_1, u_2, \ldots, u_k\}$ and $\{v_1, v_2, \ldots, v_k\}$. There must exist a node $t$ in the other component (cycle) such that $t$ is on the right of $u_0$ and $d(u_0,t) \equiv \frac{x \log n}{n}  \le \frac{a \log n}{n}$. If $x\leq b$, $\exists i \mid  i\leq k \text{ and } i(a-b)+b - a-(2i-2)\epsilon \le x\leq i(a-b)-(2i-1)\epsilon$ (see Figure~\ref{fig:arr1}). 
When $x\leq b$, we can calculate the distance between $t$ and $v_i$ as 
\begin{align*}
d(t,v_i)%& \ge d(v_i,u_0)) - d(t,u_0) \\
&\ge \frac{(i(a-b)+b-(2i-1)\epsilon)\log n}{n} - \frac{(i(a-b)-(2i-1)\epsilon) \log n}{n} = \frac{b \log n}{n}
\end{align*}
and 
\begin{align*}
d(t,v_i)%& \le d(v_i,u_0) - d(t,u_0) \\
&\le \frac{(i(a-b)+b -(2i-2)\epsilon)\log n}{n} - \frac{((i-1)(a-b)+b-a-(2i-2)\epsilon)\log n}{n} = \frac{a\log n}{n}.
\end{align*}
Therefore  $t$ is connected to $v_i$ when  $x\leq b.$ If $x >b$ then $t$ is already connected to  $u_0$. Therefore the two components (cycles) in question are connected.% when $x\ge b $ which implies that those cycles are connected. 
This is true for all cycles and hence there is only a single component in the entire graph. Indeed, if we consider the cycles to be disjoint super-nodes, then we have shown  that there must be a star configuration. % as drawn in Figure~\ref{fig:star}.
\end{proof}
%\begin{figure}
%\centering
%\begin{tikzpicture}[thick, scale=0.5]
%%\draw (-2,0) -- (2,0);
%%\filldraw [gray] (0,0) circle (4pt);
%%\draw (-2,-2) .. controls (0,0) .. (2,-2);
%%\draw (-2,2) .. controls (-1,0) and (1,0) .. (2,2);
%% \filldraw[color=black, fill=red!0,  line width=2pt](0,0) circle (3.5);
%\filldraw [gray] (0,3.5) circle (5pt);% node[anchor=north east] at (0,3.9){u};
%\filldraw [gray] (0,-3.5) circle (5pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
%\filldraw [gray] (3.5,0) circle (5pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
%\filldraw [gray] (-3.5,0) circle (5pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
%\filldraw [gray] (2.47,2.47) circle (5pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
%\filldraw [gray] (-2.47,-2.47) circle (5pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
%\filldraw [gray] (2.47,-2.47) circle (5pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
%\filldraw [gray] (-2.47,2.47) circle (5pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
%\draw [gray] (0,0) -- (0,3.5);
%\draw [gray] (0,0) -- (3.5,0);
%\draw [gray] (0,0) -- (0,-3.5);
%\draw [gray] (0,0) -- (-3.5,0);
%\draw [gray] (0,0) -- (2.47,2.47);
%\draw [gray] (0,0) -- (-2.47,-2.47);
%\draw [gray] (0,0) -- (-2.47,2.47);
%\draw [gray] (0,0) -- (2.47,-2.47);
%\filldraw [black] (0,0) circle (7pt);%node[anchor=north east] {$\frac{\beta \log n}{n}$};
%\end{tikzpicture}
%\caption{Different cycles as super-nodes connected in the form of a star, see proof of Theorem~\ref{thm:upper}.\label{fig:star}}
%\end{figure}



%To have a better understanding of how this theorem is being proved let us prove a weaker result first, and then  extend the main idea. 
%\begin{proposition}
%The random annulus graph ${\rm RAG}(n,[\frac{b\log n}{n},\frac{a\log n}{n}])$  is connected with  probability $1-o(1)$ if $a-b >1$. \label{lem:conninf}
%\end{proposition}
%\begin{proof}

%Let us determine the connectivity requirement in RAG. 

We will now provide the proof of Lemma~\ref{lem:lemma2}.

\begin{proof}[Proof of Lemma~\ref{lem:lemma2}]
Recall that we want to show that
 there exists a node $u_0$ and  $k$ nodes $\{u_1, u_2 ,\ldots, u_k\}$ to the right of $u_0$ such that $d(u_0,u_i) \in [\frac{(i(a-b)-2i\epsilon)\log n}{n},\frac{(i(a-b)-(2i-1)\epsilon) \log n}{n}]$ and exactly $k$ nodes $\{v_1, v_2 ,\ldots, v_k\}$ to the right of $u_0$ such that $d(u_0,v_i) \in [\frac{((i(a-b)+b-(2i-1)\epsilon)\log n}{n},\frac{(i(a-b)+b -(2i-2)\epsilon)\log n}{n}]$, for $i =1,2,\ldots,k$ and $\epsilon$ is a constant less than $\frac1{2k}$ (see Figure~\ref{fig:arr} for a depiction). 
 Let $A_u$ be an indicator $\{0,1\}$-random variable for every node $u$ which is $1$ if $u$ satisfies the above conditions and $0$ otherwise. We will show $\sum_{u} A_u \ge 1$ with high probability. 
 
 \begin{figure}
 \centering
 %\vspace{-20pt}
\begin{tikzpicture}[thick, scale=0.9]

\draw [gray,->] (-1,0) -- (7.5,0);
\draw [gray,dashed] (0.7,0) -- (0.7,-2);
\draw [gray,dashed] (1.7,0) -- (1.7,-2);
\draw [gray,dashed] (2.7,0) -- (2.7,-2);
\draw [gray,dashed] (3.3,0) -- (3.3,-2);
\draw [gray,dashed] (4.3,0) -- (4.3,-2);
\draw [gray,dashed] (5.3,0) -- (5.3,-1);
\draw [gray,dashed] (6.3,0) -- (6.3,-1);

\draw [green, line width=1pt] (4,0) -- (4.3,0);
\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=-2pt](4.,0) -- (4.3,0) node [black,midway,xshift=0cm,yshift=-0.31cm] {$v_1$};

\draw [green, line width=1pt] (5,0) -- (5.3,0);
\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=-2pt](5,0) -- (5.3,0) node [black,midway,xshift=0cm,yshift=-0.31cm] {$v_2$};

\draw [green, line width=1pt] (6,0) -- (6.3,0);
\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=-2pt](6,0) -- (6.3,0) node [black,midway,xshift=0cm,yshift=-0.31cm] {$v_3$};

\draw [green, line width=1pt] (0.7,0) -- (1,0);
\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=-2pt](0.7,0) -- (1,0) node [black,midway,xshift=0.1cm,yshift=-0.31cm] {$u_1$};

\draw [green, line width=1pt] (1.7,0) -- (2,0);
\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=-2pt](1.7,0) -- (2,0) node [black,midway,xshift=0.1cm,yshift=-0.31cm] {$u_2$};


\draw [green, line width=1pt] (2.7,0) -- (3,0);
\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=-2pt](2.7,0) -- (3,0) node [black,midway,xshift=0.1cm,yshift=-0.31cm] {$u_3$};

\draw [orange,<->] (-0.3,-1) -- (0.7,-1);
\draw [orange,<->] (0.7,-1) -- (1.7,-1);
\draw [orange,<->] (1.7,-1) -- (2.7,-1);
\draw [orange,<->] (4.3,-1) -- (5.3,-1);
\draw [orange,<->] (5.6,-1) -- (6.3,-1);

\draw[gray,<->] (-0.3,-2) -- node[midway,fill=white] {${a}$} (4.3,-2);
\draw[gray,<->] (-0.3,-1.5) -- node[midway,fill=white] {${b}$} (3.3,-1.5);

\draw [green, line width=1pt] (5.7,3) -- (6,3)node [black,midway,xshift=0.4cm,yshift=0cm] {$\epsilon$};
\draw [orange,<->] (5.7,2.5) -- (6,2.5)node [black,midway,xshift=1cm,yshift=0cm] {$a-b-2\epsilon$};

%\filldraw [gray] (3.5,0) circle (5pt);%node[anchor=south] at (3.5,-1) {$\frac{a\log n}{n}$};;% node[anchor=north east] at (0,3.9){u};
%\filldraw [gray] (-3.5,0) circle (5pt);%node[anchor=south] at (-3.5,-1) {$-\frac{a\log n}{n}$};;%node[anchor=north east] {$\frac{\beta \log n}{n}$};
%\filldraw [gray] (-2.5,0) circle (5pt);%node[anchor=south] at (-2.5,-1) {$-\frac{b\log n}{n}$};;%node[anchor=north east] {$\frac{\beta \log n}{n}$};
%\filldraw [gray] (2.5,0) circle (5pt);%node[anchor=south] at (2.5,-1) {$\frac{b\log n}{n}$};;%node[anchor=north east] {$\frac{\beta \log n}{n}$};

\draw[blue]    (-0.3,0) to[out=40,in=140,distance=3cm](4.15,0) ;
\draw[blue]    (0.85,0) to[out=40,in=140,distance=2cm](4.15,0) ;
\draw[red]    (0.85,0) to[out=40,in=140,distance=3cm](5.15,0) ;
\draw[red]    (1.85,0) to[out=40,in=140,distance=2cm](5.15,0) ;
\draw[violet]    (1.85,0) to[out=40,in=140,distance=3cm](6.15,0) ;
\draw[violet]    (2.85,0) to[out=40,in=140,distance=2cm](6.15,0) ;


\filldraw [black] (-0.3,0) circle (5pt)node[anchor=south] at (0,-0.6) {$u_0$};
\end{tikzpicture}
\caption{The location of $u_i$ and $v_i$ relative to $u$ scaled by $\frac{\log n}{n}$ in Lemma \ref{lem:lemma2}. Edges stemming put of  $v_1,v_2, v_3$ are shown as blue, red and violet respectively. \label{fig:arr}}
\end{figure}
 
 
 We  have,
\begin{align*}
\Pr(A_u=1) & = n(n-1)\dots (n-(2k-1))\Big(\frac{\epsilon \log n}{2\pi n}\Big)^{2k} \Big(1-2k\epsilon \frac{\log n}{2\pi n}\Big)^{n-2k}\\
%(2k)!\binom{n}{2k} \Big(\frac{\epsilon \log n}{n}\Big)^{2k} \Big(1-2k\epsilon \frac{\log n}{n}\Big)^{n-2k}\\&=\Big(1-2k\epsilon \frac{\log n}{n}\Big)^{n-1}\prod_{i=1}^{2k}(n -(i-1))\Big(\frac{\epsilon \log n}{n}\Big)\Big(1-2k\epsilon \frac{\log n}{n}\Big)^{-1}\\
%& = \Big(1-2k\epsilon \frac{\log n}{n}\Big)^{n-2k}  \prod_{i=0}^{2k-1} (n-i)\frac{\epsilon \log n}{n}\\
& = c_0 n^{-2k\epsilon} (\epsilon/2\pi \log n)^{2k}  \prod_{i=0}^{2k-1} (1-i/n)\\
&= c_1 n^{-2k\epsilon} (\epsilon/2\pi \log n)^{2k}
\end{align*}
where $c_0,c_1$ are just absolute constants independent of $n$ (recall $k$ is a constant). %$ \prod_{i=0}^{2k-1} (1-i/n) \rightarrow 1$ as $n \rightarrow \infty$ and $k$ is just a constant. 
Hence,
\begin{align*}
\sum_{u} \avg A_u= c_1 n^{1-k\epsilon/\pi} (\epsilon \log n)^{2k} \ge 1
\end{align*} 
as long as $\epsilon \leq \frac{\pi}{2k}$.  Now, in order to prove $\sum_{u}  A_u\ge 1$ with high probability, we will show that the variance of $\sum_{u}  A_u$  is bounded from above.  This calculation is very similar to the one in the proof of Theorem~\ref{thm:lower_bound}. 
Recall that if $A =\sum_{u}  A_u$ is a sum of indicator random variables, we must have 
$${\rm Var}(A) \le \avg[A]+\sum_{u \neq v} {\rm Cov}(A_u,A_v)=\avg[A]+\sum_{u \neq v} \Pr(A_u=1 \cap A_v=1)-\Pr(A_u=1)\Pr(A_v=1).$$ 
Now first consider the case when vertices $u$ and $v$ are at a distance of at least $\frac{2(a+b) \log n}{n}$ apart (happens with probability $1- \frac{4(a+b)\log n}{2\pi n}$). 
Then the region in $[0,2\pi]$ that is within distance $\frac{(a+b)\log n}{n}$ from both $u$ and $v$ is the empty-set. In this case, $\Pr(A_u=1 \cap A_v=1) = n(n-1)\dots (n-(4k-1))\Big(\frac{\epsilon \log n}{2\pi n}\Big)^{4k} \Big(1-4k\epsilon \frac{\log n}{2\pi n}\Big)^{n-4k} = c_2 n^{-2k\epsilon/\pi} (\epsilon/2\pi \log n)^{4k},$ where $c_2$ is a constant.

In all other cases, $\Pr(A_u=1 \cap A_v=1) \le \Pr(A_u =1)$.
%then their corresponding regions of interest i.e the regions which are at a distance of $[0,r_s]$ away from their respective nodes are disjoint and hence the random variables $A_u$ and $A_v$ are asymptotically independent (since $k$ is just a constant). 
Therefore,
%Otherwise we can upper bound the probability $\Pr(A_u=1 \cap A_v=1)$ by taking the regions of interest to be the same. Hence, we have that  
\begin{align*}
\Pr(A_u=1 \cap A_v=1)=\Big(1-\frac{4(a+b) \log n}{2\pi n}\Big) c_2 n^{-2k\epsilon/\pi} (\epsilon/2\pi \log n)^{4k}+ \frac{4(a+b) \log n}{2\pi n} c_1n^{-k\epsilon/\pi} (\epsilon/2\pi \log n)^{2k} 
\end{align*}
and
\begin{align*}
{\rm Var(A)} &\le c_1n^{1-k\epsilon/\pi} (\epsilon/2\pi \log n)^{2k} +{n \choose 2}\Big(\Pr(A_u=1 \cap A_v=1)-\Pr(A_u=1)\Pr(A_v=1)\Big) \\
&\le c_1n^{1-k\epsilon/\pi} (\epsilon/2\pi \log n)^{2k}+ c_3 n^{1-k\epsilon/\pi} (\log n)^{2k+1}\\
& \le c_4  n^{1-k\epsilon/\pi} (\log n)^{2k+1}
\end{align*}
where $c_3,c_4$ are constants. Again invoking Chebyshev's inequality, with probability at least $1-\frac{1}{\log n}$ 
$$
A > c_1n^{1-k\epsilon/\pi} (\epsilon/2\pi \log n)^{2k} - \sqrt{c_4  n^{1-k\epsilon/\pi} (\log n)^{2k+2}}.
$$  

\end{proof}

\begin{figure}
\centering
\begin{tikzpicture}[thick, scale=0.9]

\draw [gray,->] (-1,0) -- (10.5,0);
\draw [gray,dashed] (0.7,0.3) -- (0.7,-2);
\draw [gray,dashed] (1.7,0.7) -- (1.7,-2);
\draw [gray,dashed] (2,0.35) -- (2,0);
\draw [gray,dashed] (3,0.7) -- (3,0);
\draw [gray,dashed] (2.7,0) -- (2.7,-2);
\draw [gray,dashed] (3.3,0) -- (3.3,-2);
\draw [gray,dashed] (4.3,0) -- (4.3,-2);
\draw [gray,dashed] (5.3,0) -- (5.3,-1);
\draw [gray,dashed] (6.3,0) -- (6.3,-1);

\draw [blue, line width=1pt] (4,0) -- (4.3,0);
\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=-2pt](4.,0) -- (4.3,0) node [black,midway,xshift=0cm,yshift=-0.31cm] {$v_1$};

\draw [blue, line width=1pt] (5,0) -- (5.3,0);
\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=-2pt](5,0) -- (5.3,0) node [black,midway,xshift=0cm,yshift=-0.31cm] {$v_2$};

\draw [blue, line width=1pt] (6,0) -- (6.3,0);
\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=-2pt](6,0) -- (6.3,0) node [black,midway,xshift=0cm,yshift=-0.31cm] {$v_3$};

\draw [blue, line width=1pt] (0.7,0) -- (1,0);
%\draw [blue, line width=2pt] (-0.3,-0.05) -- (1,-0.05);
\draw [blue,decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=-2pt](-0.3,0.1) -- (1,0.1);% node [black,midway,xshift=0.1cm,yshift=-0.31cm] {$u_1$};
\draw [red,decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=-2pt](.7,0.4) -- (2,0.4);% node [black,midway,xshift=0.1cm,yshift=-0.31cm] {$u_1$};
\draw [violet,decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=-2pt](1.7,0.8) -- (3,0.8);% node [black,midway,xshift=0.1cm,yshift=-0.31cm] {$u_1$};
%\draw [blue, line width=2pt] (0.7,-0.1) -- (2,-0.1);
%\draw [blue, line width=2pt] (1.7,-0.15) -- (3,-0.15);


\draw [blue, line width=1pt] (1.7,0) -- (2,0);
%\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=-2pt](1.7,0) -- (2,0) node [black,midway,xshift=0.1cm,yshift=-0.31cm] {$u_2$};


\draw [blue, line width=1pt] (2.7,0) -- (3,0);
%\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=-2pt](2.7,0) -- (3,0) node [black,midway,xshift=0.1cm,yshift=-0.31cm] {$u_3$};

\draw [orange,<->] (-0.3,-1) -- (0.7,-1);
\draw [orange,<->] (0.7,-1) -- (1.7,-1);
\draw [orange,<->] (1.7,-1) -- (2.7,-1);
\draw [orange,<->] (4.3,-1) -- (5.3,-1);
\draw [orange,<->] (5.6,-1) -- (6.3,-1);

\draw[gray,<->] (-0.3,-2) -- node[midway,fill=white] {${a}$} (4.3,-2);
\draw[gray,<->] (-0.3,-1.5) -- node[midway,fill=white] {${b}$} (3.3,-1.5);

\draw [blue, line width=1pt] (5.7,3) -- (6,3)node [black,midway,xshift=0.4cm,yshift=0cm] {$\epsilon$};
\draw [orange,<->] (5.7,2.5) -- (6,2.5)node [black,midway,xshift=1cm,yshift=0cm] {$a-b-2\epsilon$};

%\filldraw [gray] (3.5,0) circle (5pt);%node[anchor=south] at (3.5,-1) {$\frac{a\log n}{n}$};;% node[anchor=north east] at (0,3.9){u};
%\filldraw [gray] (-3.5,0) circle (5pt);%node[anchor=south] at (-3.5,-1) {$-\frac{a\log n}{n}$};;%node[anchor=north east] {$\frac{\beta \log n}{n}$};
%\filldraw [gray] (-2.5,0) circle (5pt);%node[anchor=south] at (-2.5,-1) {$-\frac{b\log n}{n}$};;%node[anchor=north east] {$\frac{\beta \log n}{n}$};
%\filldraw [gray] (2.5,0) circle (5pt);%node[anchor=south] at (2.5,-1) {$\frac{b\log n}{n}$};;%node[anchor=north east] {$\frac{\beta \log n}{n}$};

\draw[blue]    (0.35,0.17) to[out=40,in=140,distance=2cm](4.15,0) ;
%\draw[blue]    (0.85,0) to[out=40,in=140,distance=2cm](4.15,0) ;
\draw[red]    (1.3,0.4) to[out=50,in=140,distance=3cm](5.15,0) ;
%\draw[red]    (1.85,0) to[out=40,in=140,distance=2cm](5.15,0) ;
%\draw[violet]    (1.85,0) to[out=40,in=140,distance=3cm](6.15,0) ;

\draw[violet]    (2.3,0.8) to[out=40,in=140,distance=2cm](6.15,0) ;


\filldraw [black] (-0.3,0) circle (5pt)node[anchor=south] at (-0.5,-0.6) {$u$};
\end{tikzpicture}
\caption{The line segments where $v_1,v_2,v_3$ can have neighbors (scaled by $\frac{\log n}{n}$) in the proof of Theorem \ref{thm:upper}. The point $t$ has to lie in one of these regions.\label{fig:arr1}}
\end{figure}

It remains to prove Lemma~\ref{lem:lemma1}. 
 
 \begin{proof}[Proof of Lemma~\ref{lem:lemma1}]
 The proof of this lemma is somewhat easily explained if we consider a weaker result (a stronger condition) with $a -b >4\pi/3$. Let us first briefly describe this case.


Consider a node $u$ and assume without loss of generality that the position of $u$ is $0$ (i.e. $X_u=0$). Associate four indicator $\{0,1\}$-random variables $A_u^i, i =1,2,3,4$ which take the value of $1$ if and only if there does not exist any node $x$ such that 
\begin{enumerate}
\item $d(u,x) \in [b\frac{\log n}{n},a\frac{\log n}{n}] \cup [0,\frac{a-b}{2}\frac{\log n}{n}]\} \text{  for  } i=1$
\item $d(u,x) \in [b\frac{\log n}{n},a\frac{\log n}{n}] \cup [-b\frac{\log n}{n},\frac{-a-b}{2}\frac{\log n}{n}]\}  \text{  for  } i=2$
\item $d(u,x) \in [-b\frac{\log n}{n},-a\frac{\log n}{n}] \cup [\frac{-a+b}{2}\frac{\log n}{n},0]\}  \text{  for  } i=3$
\item $d(u,x) \in [-b\frac{\log n}{n},-a\frac{\log n}{n}] \cup [b\frac{\log n}{n},\frac{a+b}{2}\frac{\log n}{n}]\}  \text{  for  } i=4.$
\end{enumerate}
The intervals representing these random variables are shown in Figure~\ref{fig:four}.

Notice that $\Pr(A^i_u=1)=\max\{\Big(1-1.5(a-b)\frac{\log n}{2\pi n}\Big)^{n-1},\Big(1-a\frac{\log n}{2\pi n}\Big)^{n-1}\}$ and therefore $\sum_{i,u} \avg A^i_u \approx 4\max\{n^{1-\frac{1.5(a-b)}{2\pi}},n^{1-\frac{a}{2\pi}}\}$.  This means that for $a-b \ge \frac{4\pi}{3}$ and $a \ge 2\pi$, $\sum_{i,u} \avg A^i_u=o(1)$.  Hence there exist vertices in all the regions described above for every node $u$ with high  probability.
 
%Observe that the constraint $\alpha<3\beta$ results in the regions $[0,\frac{\alpha-\beta}{2}\frac{\log n}{n}],[-\beta\frac{\log n}{n},\frac{-\alpha-\beta}{2}\frac{\log n}{n}],[\frac{-\alpha+\beta}{2}\frac{\log n}{n},0]$ and $[\beta\frac{\log n}{n},\frac{\alpha+\beta}{2}\frac{\log n}{n}]$ to have no overlap and therefore they are disjoint regions. 
Now, $A_u^1$ and $A_u^2$ being zero implies that either there is a vertex in $ [b\frac{\log n}{n},a\frac{\log n}{n}] $ or there exists two vertices $v_1,v_2$ in $ [0,\frac{a-b}{2}\frac{\log n}{n}]$ and $[-b\frac{\log n}{n},\frac{-a-b}{2}\frac{\log n}{n}]$ respectively (see, Figure~\ref{fig:four}). In the second case, $u$ is connected to $v_2$ and $v_2$ is connected to $v_1$. Therefore $u$ has nodes on left ($v_2$) and right ($v_1$) and $u$ is connected to both of them through one hop in the graph. 

Similarly, $A_u^3$ and $A_u^4$ being zero implies that either there exists a vertex in $[-b\frac{\log n}{n},-a\frac{\log n}{n}]$ or again $u$ will have vertices on left and right and will be connected to them. So , when all the four $A_u^i, i=1,2,3,4$ are zero together, the only exceptional case is when there are nodes in $[b\frac{\log n}{n},a\frac{\log n}{n}] \}$ and $[-b\frac{\log n}{n},-a\frac{\log n}{n}]$. But in that case $u$ has direct neighbors on both its left and right. %So we can conclude that for 
%every node $u$, there exists a node $v$ such that $d(u,v) \in [0,a \frac{\log n}{n}]$ and a node $w$ such that $d(u,w) \in [-a\frac{\log n}{n},0]$ and $u,v,w$ are connected. This implies that
We can conclude that every vertex $u$ is connected to  a vertex  $v$ on  its right and a vertex  $w$ on its left  such that $d(u,v) \in [0,a \frac{\log n}{n}]$ and  $d(u,w) \in [-a\frac{\log n}{n},0]$; therefore every vertex is part of a cycle that covers $[0,2\pi]$.

 \begin{figure}
   \centering
\begin{tikzpicture}[thick, scale=0.9]
\draw [gray,<->] (0,1.5) -- (0.5,1.5)node at (1,1.5) {$\frac{a-b}{2}$};;
\draw[pattern=north west lines,pattern color=red][preaction={fill=blue!20}] (3.5,1.9) -- (4.5,1.9) -- (4.5,1.7) -- (3.5,1.7) -- cycle node at (4.8,1.8) {$A_u^3$};;
\draw[pattern=vertical lines,pattern color=red][preaction={fill=blue!50}]  (3.5,1.4) -- (4.5,1.4) -- (4.5,1.2) -- (3.5,1.2) -- cycle node at (4.8,1.2) {$A_u^4$};;
\draw[pattern=dots,pattern color=blue] [preaction={fill=gray}]  (1.5,1.9) -- (2.5,1.9) -- (2.5,1.7) -- (1.5,1.7) -- cycle node at (2.8,1.8) {$A_u^1$};;
\draw[pattern=grid,pattern color=violet][preaction={fill=red!50}]   (1.5,1.4) -- (2.5,1.4) -- (2.5,1.2) -- (1.5,1.2) -- cycle node at (2.8,1.2) {$A_u^2$};;

\draw[pattern=dots,pattern color=blue][preaction={fill=gray}]  (3.5,0) -- (4.5,0) -- (4.5,-0.3) -- (3.5,-0.3) -- cycle;
\draw[pattern=grid,pattern color=violet] [preaction={fill=red!50}]  (3.5,-0.3) -- (4.5,-0.3) -- (4.5,-0.6) -- (3.5,-0.6) -- cycle;
\draw[pattern=north west lines,pattern color=red][preaction={fill=blue!20}]  (-3.5,0) -- (-4.5,0) -- (-4.5,-0.3) -- (-3.5,-0.3) -- cycle;
\draw[pattern=vertical lines,pattern color=red][preaction={fill=blue!50}]   (-3.5,-0.3) -- (-4.5,-0.3) -- (-4.5,-0.6) -- (-3.5,-0.6) -- cycle;
\draw[pattern=dots,pattern color=blue][preaction={fill=gray}]  (0,0) -- (.5,0) -- (.5,-0.3) -- (0,-0.3) -- cycle;
\draw[pattern=north west lines,pattern color=red][preaction={fill=blue!20}]  (0,0) -- (-.5,0) -- (-.5,-0.3) -- (0,-0.3) -- cycle;
\draw[pattern=vertical lines,pattern color=red][preaction={fill=blue!50}]   (3.5,-0.6) -- (4,-0.6) -- (4,-0.9) -- (3.5,-0.9) -- cycle;
\draw[pattern=grid,pattern color=violet] [preaction={fill=red!50}]  (-3.5,0) -- (-3,0) -- (-3,-0.3) -- (-3.5,-0.3) -- cycle;

%\draw [gray,<->] (-3.5,-1.3) -- (-4.5,-1.3);
%\draw [gray,<->] (3.5,-1.3) -- (4.5,-1.3);
\draw [gray,<->] (3.5,-1.3) -- (4,-1.3);
\draw [gray,<->] (0,-1.3) -- (0.5,-1.3);
\draw [gray,<->] (0,-1.3) -- (-.5,-1.3);
\draw [gray,<->] (-3.5,-1.3) -- (-3,-1.3);



%
%
\draw [gray,<->] (-5,0) -- (5,0);
\draw [gray,dashed] (3.5,0) -- (3.5,-1.4);
%\draw [gray,dashed] (4.5,0) -- (4.5,-1.4);
\draw [gray,dashed] (0.5,0) -- (0.5,-1.4);
\draw [gray,dashed] (0,0) -- (0,-1.4);
\draw [gray,dashed] (-0.5,0) -- (-0.5,-1.4);
\draw [gray,dashed] (-3.5,0) -- (-3.5,-1.4);
%\draw [gray,dashed] (-4.5,0) -- (-4.5,-1.4);
\draw [gray,dashed] (-3,0) -- (-3,-1.4);
\draw [gray,dashed] (4,0) -- (4,-1.4);
\draw node[anchor=south] at (3.5,0) {$b$};
\draw node[anchor=south] at (4.5,0) {$a$};
\draw node[anchor=south] at (-3.5,0) {$-b$};
\draw node[anchor=south] at (-4.5,0) {$-a$};

%\draw [blue, line width=1pt,<->] (3.5,-0.5) -- (4.5,-0.5);
%\draw [blue, line width=1pt,<->] (0,-0.5) -- (0.5,-0.5);
%
%\draw [violet, line width=1pt,<->] (3.5,-0.8) -- (4.5,-0.8);
%\draw [violet, line width=1pt,<->] (-3.5,-0.8) -- (-3,-0.8);
%
%\draw [red, line width=1pt,<->] (-3.5,-1.1) -- (-4.5,-1.1);
%\draw [red, line width=1pt,<->] (0,-1.1) -- (-0.5,-1.1);
%
%
%\draw [green, line width=1pt,<->] (3.5,-1.4) -- (4,-1.4);
%\draw [green, line width=1pt,<->] (-3.5,-1.4) -- (-4.5,-1.4);
\filldraw [black] (0,0) circle (3pt)node[anchor=south] at (0,0) {$u$};
\end{tikzpicture}
\caption{Representation of four different random variables for Lemma \ref{lem:lemma1}. \label{fig:four}}
\end{figure}

We can  now extend this proof to the case when $a-b> \pi.$
%\begin{lemma}
%For any constant $c$, the Random Annulus Graph $G(n,[\frac{a \log n}{n},\frac{b \log n}{n}])$ is connected if $a-b \ge \frac{2^{c}}{2^{c+1}-1}$ and $a\ge 1$
%\end{lemma}

Let $c$ be large number to  be chosen specifically later.
Consider a node $u$ and assume that the position of $u$ is $0$. Now consider the three different regions (as defined below)  $u$ each divided into $L\equiv 2^{c}$ patches (intervals) of size $\theta=\frac{a-b}{2^c}$  in  the following way:
\begin{enumerate}
\item $I_u^i=[\frac{(-a + (i-1)\theta )\log n}{n},\frac{(-a + i\theta)  \log n}{n}]$
\item $J_u^i=[\frac{(-(a-b) + (i-1)\theta )\log n}{n},\frac{(-(a-b) + i\theta)  \log n}{n}]$
\item $K_u^i= [\frac{(b + (i-1)\theta )\log n}{n},\frac{(b + i\theta)  \log n}{n}]$
\item $M_u^i= [\frac{( (i-1)\theta )\log n}{n},\frac{ i\theta  \log n}{n}]$
\end{enumerate}
where $i=1,2,3,\ldots,L$. Note that any vertex in $\cup I_u^i \cup K_u^i$ is connected to $u$. See, Figure~\ref{fig:patch} for a depiction.



\begin{figure}
\centering
\begin{tikzpicture}[thick, scale=0.9]
\draw [gray,<->] (-5,0) -- (5,0);\filldraw [black] (0,0) circle (3pt)node[anchor=south] at (0.1,-0.7) {$u$};
\draw[<->] (0,-1.1) -- node[midway,fill=white] {$a-b$} (-1,-1.1);
\draw[<->] (0,-1.1) -- node[midway,fill=white] {$a-b$} (1,-1.1);
\draw[<->] (0,-1.35) -- node[midway,fill=white] {$b$} (-3.5,-1.35);
\draw[<->] (0,-1.7) -- node[midway,fill=white] {$a$} (-4.5,-1.7);
\draw[<->] (0,-1.35) -- node[midway,fill=white] {$b$} (3.5,-1.35);
\draw[<->] (0,-1.7) -- node[midway,fill=white] {$a$} (4.5,-1.7);


\draw [blue, line width=1pt] (-4.5,0) -- (-4.25,0);
\draw [blue, line width=1pt] (-4.25,0) -- (-4,0);
\draw [blue, line width=1pt] (-4,0) -- (-3.75,0);
\draw [blue, line width=1pt] (-3.75,0) -- (-3.5,0);

\draw [blue, line width=1pt] (-2.00,1) -- (-2.25,1) node [black,midway,xshift=0.4cm,yshift=0cm] {$\theta$};;
\draw [gray] (-2.00,1.2) -- (-2.00,0.8);
\draw [gray] (-2.25,1.2) -- (-2.25,0.8);

\draw [gray] (4.5,0.2) -- (4.5,-.2);
\draw [gray] (4.25,0.2) -- (4.25,-.2);
\draw [gray] (4,0.2) -- (4,-.2);
\draw [gray] (3.75,0.2) -- (3.75,-.2);
\draw [gray] (3.5,0.2) -- (3.5,-.2);


\draw [gray] (-4.5,0.2) -- (-4.5,-.2);
\draw [gray] (-4.25,0.2) -- (-4.25,-.2);
\draw [gray] (-4,0.2) -- (-4,-.2);
\draw [gray] (-3.75,0.2) -- (-3.75,-.2);
\draw [gray] (-3.5,0.2) -- (-3.5,-.2);


\draw [gray] (-1,0.2) -- (-1,-.2);
\draw [gray] (-.75,0.2) -- (-.75,-.2);
\draw [gray] (-0.5,0.2) -- (-0.5,-.2);
\draw [gray] (-.25,0.2) -- (-.25,-.2);
\draw [gray] (0,0.2) -- (0,-.2);
\draw [gray] (1,0.2) -- (1,-.2);
\draw [gray] (.75,0.2) -- (.75,-.2);
\draw [gray] (0.5,0.2) -- (0.5,-.2);
\draw [gray] (.25,0.2) -- (.25,-.2);
\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=0pt](3.5,-0.2) -- (4.5,-0.2) node [black,midway,xshift=0cm,yshift=-0.4cm] {$K_u^i$};
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt](0,-0.2) -- (-1,-0.2) node [black,midway,xshift=0cm,yshift=-0.4cm] {$J_u^i$};
\draw [decorate,decoration={brace,amplitude=3pt,mirror},xshift=0pt,yshift=0pt](0,-0.2) -- (1,-0.2) node [black,midway,xshift=0cm,yshift=-0.4cm] {$M_u^i$};

\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt](-3.5,-0.2) -- (-4.5,-0.2) node [black,midway,xshift=0cm,yshift=-0.4cm] {$I_u^i$};
%\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=-2pt](4.25,-0) -- (4,-0) node [black,midway,xshift=0cm,yshift=-0.3cm] {$C_u^1$};
%\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=-2pt](4,-0) -- (3.75,-0) node [black,midway,xshift=0cm,yshift=-0.3cm] {$C_u^1$};
%\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=-2pt](3.75,-0) -- (3.5,-0) node [black,midway,xshift=0cm,yshift=-0.3cm] {$C_u^1$};

\draw [blue, line width=1pt] (-1,0) -- (-0.75,0);
\draw [blue, line width=1pt] (-0.75,0) -- (-0.5,0);
\draw [blue, line width=1pt] (-0.5,0) -- (-0.25,0);
\draw [blue, line width=1pt] (-0.25,0) -- (0,0);

\draw [blue, line width=1pt] (1,0) -- (0.75,0);
\draw [blue, line width=1pt] (0.75,0) -- (0.5,0);
\draw [blue, line width=1pt] (0.5,0) -- (0.25,0);
\draw [blue, line width=1pt] (0.25,0) -- (0,0);


\draw [blue, line width=1pt] (4.5,0) -- (4.25,0);
\draw [blue, line width=1pt] (4.25,0) -- (4,0);
\draw [blue, line width=1pt] (4,0) -- (3.75,0);
\draw [blue, line width=1pt] (3.75,0) -- (3.5,0);


\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt](3.5,0.2) -- (3.75,0.2);% node [black,midway,xshift=0cm,yshift=0.4cm] {$A_u^i$};
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt](3.75,0.2) -- (4,0.2);% node [black,midway,xshift=0cm,yshift=0.4cm] {$A_u^i$};
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt](4,0.2) -- (4.25,0.2);% node [black,midway,xshift=0cm,yshift=0.4cm] {$A_u^i$};
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt](-0.75,0.2) -- (-0.5,0.2);% node [black,midway,xshift=0cm,yshift=0.4cm] {$A_u^i$};
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt](-0.5,0.2) -- (-0.25,0.2);% node [black,midway,xshift=0cm,yshift=0.4cm] {$A_u^i$};
\draw [decorate,decoration={brace,amplitude=3pt},xshift=0pt,yshift=0pt](-0.25,0.2) -- (0,0.2);% node [black,midway,xshift=0cm,yshift=0.4cm] {$A_u^i$};


\draw[blue]    (-0.125,0.3) to[out=60,in=120,distance=1cm](3.625,0.3) ;
\draw[blue]    (-0.125,0.3) to[out=60,in=120,distance=1cm](3.875,0.3) ;
\draw[blue]    (-0.125,0.3) to[out=60,in=120,distance=1cm](4.125,0.3) ;


\draw[red]    (-0.375,0.3) to[out=60,in=120,distance=2cm](3.875,0.3) ;
\draw[red]    (-0.375,0.3) to[out=60,in=120,distance=2cm](3.625,0.3) ;

\draw[violet]    (-0.625,0.3) to[out=60,in=120,distance=3cm](3.625,0.3) ;

\end{tikzpicture}
\caption{Pictorial representation of $I_u^i, J_u^i, K_u^i, M_u^i$ and their connectivity as described in Lemma \ref{lem:lemma1}. The colored lines show the regions that are connected to each other.\label{fig:patch}}
\end{figure}


Consider a $\{0,1\}$-indicator random variable $X_u$ that is $1$ if and only if there does not exist any node in some region that consists of $2L-1$ patches amongst the ones described above. Notice that if the patches do not overlap then the total size of $2L-1$ patches is $\frac{2^{c+1}-1}{2^c}\frac{(a-b)\log n}{n}$ and if they do overlap, then the total size of the $2L-1$ patches is going to be less than $\min\{\frac{2^{c+1}-1}{2^c}\frac{(a-b)\log n}{n},\frac{a \log n}{n}\}$. 
%Define the $\{0,1\}$-indicator random variable $Y$ which is $1$ if and only if there does not exist any node in a particular region consisting of $2L-1$ patches. Therefore, $\Pr(Y=1) \le \max\{\Big(1-\frac{2^{c+1}-1}{2^c}\frac{(a-b)\log n}{n}\Big)^{n},\Big(1-\frac{a\log n}{n}\Big)^{n}\}$. 
Since there are ${4L \choose 2L-1}\le n^{\frac{4L}{\log n}}$ possible regions that consists of $2L-1$ patches, 
\begin{align*}
 \sum_u \avg X_u &\leq n {4L \choose 2L-1}\Big(1-\min\{\frac{2^{c+1}-1}{2^c}\frac{(a-b)\log n}{2\pi n},\frac{a \log n}{2\pi n}\}\Big)^{n-1}\\
 & \le \max\{n^{1-\frac{2^{c+1}-1}{2^c}\frac{(a-b)}{2\pi} +\frac{4L}{\log n}}, n^{1-\frac{a}{2\pi}+\frac{4L}{\log n}}\}.
 %\max\{n^{1-\frac{2^{c+1}-1}{2^c}(a-b)},n^{1-a}\}.
\end{align*}
At this point we can choose $c= c_n = o(\log n)$ such that $\lim_n c_n = \infty$.
 Hence when $a-b > {\pi}$ %\frac{2^c}{2^{c+1}-1}$ 
 and $a > 2\pi$, for every vertex $u$ there exists at least one patch amongst every $2L-1$ patches in $\cup I_u^i \cup J_u^j \cup K_u^k, i,j,k =1,2, \dots, L$ that contains a vertex.


Consider a collection of patches $\cup_iI_u^i \cup_j J_u^j,  i,j=1, 2, \dots, L$. We know that there exist two patches amongst these $I_u^i$s and $K_u^j$s that contain at least one vertices. If one of $I_u^i$s and one of $K_u^j$s contain two vertices, we found one neighbor of $u$ on both left and right directions (see, Figure~\ref{fig:patch}).


We consider the other case now.
Without loss of generality assume that there are no vertex in all $I_u^i$s and there exist at least two patches in $K_u^i$s that contain at least one vertex each. Hence, there exists at least one of $\{K_u^i \mid i\in \{1,2, \ldots, L-1\}\}$ that contains a vertex. Similarly, we can also conclude in this case that there exists at least one of $\{J_u^i \mid i\in \{2,3 \ldots, L\}\}$ which contain a node. Assume $J_u^{\phi}$ to be the left most patch in $\cup J_u^i \mid i \in \{1, 2, \dots, L\}$ that contains a vertex (see,Figure~\ref{fig:patch}) . From our previous observation, we can conclude that $\phi \ge 2$. 



We can observe that any vertex in $J_u^j$ is connected to the vertices in patches $K_u^k,  \forall k<j$. 
This is because for two vertices $v\in J_u^j$ and $w\in K_u^k$, we have
\begin{align*}
d(v,w) &\ge \frac{(b + (k-1)\theta )\log n}{n} - \frac{(-(a-b) + j\theta)  \log n}{n}
= \frac{(a + (k-j-1)\theta )\log n}{n}; \\
d(v,w) &\le \frac{(b + k\theta)  \log n}{n} - \frac{(-(a-b) + (j-1)\theta )\log n}{n}
= \frac{(a + (k-j+1)\theta )\log n}{n}. 
\end{align*}

%If there exists a node in $B^{|L|}_u$, then it is connected to the node in $C_u^i \ \forall i\in{1,2,\ldots, |L|-1}$. If this is not the case, then
%If there doesnt exist a node in $B_{|L|}$ but a node in $B_{|L|-1}$ then it is connected to all nodes in $C_i \ \forall i\in\{1,2,\ldots |L|-1\}$. Consider the set $B_|L| \cup A_i \cup C_{j}\forall i\in L, \ j\in\{1,2,3,\ldots, |L|-1\}$ which consists of a collection of $2|L|-1$ patches. Since atleast one of these patch must have a node and none of $A_i$ of $B_{|L|}$ can contain a node. Hence, node in $B_{|L|-1}$ is connected to the node in $C_j$ which is connected to $u$.Considering just $A_i$, $B_j$,  $\forall i\ge 1,j\ge2$, there exists atleast one node in $B_j$, $j\ge2$. Additionally, if there does not exist a node in all $B_j$'s $\forall j > \phi $, 


Consider a collection of $2L-1$ patches $\{\cup I_u^i  \cup J_u^j \cup K_u^k \mid i,j,k\in \{1,\dots, L\}, j>\phi, k\le \phi-1\}$ where $\phi \ge 2$. This is a collection of $2L-1$ patches out of which one must have a vertex and since none of $\{J_u^j \mid j>\phi\}$ and $I_u^i$ can contain a vertex, one of $\{K_u^k \mid k \le \phi -1\}$  must contain the vertex. Recall that the vertex in $J_u^{\phi}$ is connected to any node in $K_u^k$ for any $k\le \phi-1$ and therefore $u$ has a node to the right direction and left direction that are connected to $u$. Therefore every vertex is part of a cycle and each of the circles  covers $[0,2\pi]$.
 \end{proof}



The following result is an immediate corollary of the connectivity upper bound.
\begin{corollary}\label{cor:patch}
Consider a random  graph $G(V,E)$  is being  generated as a variant of the RAG where each  $u,v\in V$ forms an edge if and only if  $d(u,v)\in \left[0,c\frac{\log n}{n}\right]\cup \left[b\frac{\log n}{n},a\frac{\log n}{n}\right], 0 <c<b<a$. This graph is connected with  probability $1-o(1)$ if $a-b + c>2\pi$ or if $a-b > \pi, a>2\pi$. \label{cor:patches}
\end{corollary}

The above corollary can be further improved for some regimes of $a,b,c$. In particular, we can get the following result (proof delegated to  the appendix).

\begin{corollary}\label{cor:extra}
Consider a random  graph $G(V,E)$  is being  generated as a variant of the RAG where each  $u,v\in V$ forms an edge if and only if  $d(u,v)\in \left[0,c\frac{\log n}{n}\right]\cup \left[b\frac{\log n}{n},a\frac{\log n}{n}\right], 0 <c<b<a$. This graph is connected with  probability $1-o(1)$ if
either of the following conditions are true:
\begin{enumerate}
\item $2(a-b)+ c/2 > 2\pi \text{ when } a-b<c \text{ and }b>3c/2$
\item $b-c > 2\pi \text{ when } a-b<c \text{ and }b\le 3c/2$
\item $a > 2\pi \text{ when } a-b\ge c \text{ and } b\le 3c/2 $
\item $(a-b)+ 3c/2  > 2\pi \text{ when } a-b\ge c \text{ and } b>3c/2$.
\end{enumerate}
\end{corollary}


\subsection{Necessary condition for connectivity of RAG}

\begin{theorem}[RAG connectivity lower bound]\label{thm:lower_bound}
The ${\rm RAG}(n,[\frac{b\log n}{n},\frac{a\log n}{n}])$  is not connected
with  probability $1-o(1)$ if $a <	2\pi$ or $a-b < \pi$. 
%
\end{theorem}
\begin{proof}
First of all,  it is known that ${\rm RAG}(n,[0,\frac{a\log n}{n}])$ (which is the random geometric graph ${\rm RGG}(n, \frac{a\log n}{n})$) is not connected  with  high probability when $a <2\pi$ \citep{muthukrishnan2005bin,penrose2003random} (The original papers have a threshold of 1 assuming the radius is $\frac{1}{2\pi}$. We prove this threshold with our technique in Lemma \ref{lem:rgglower}). Therefore  ${\rm RAG}(n,[\frac{b\log n}{n},\frac{a\log n}{n}])$ must not be connected with high probability when $a<2\pi$ as the connectivity interval is a strict subset of the previous case, and ${\rm RAG}(n,[\frac{b\log n}{n},\frac{a\log n}{n}])$ can be obtained from ${\rm RAG}(n,[0,\frac{a\log n}{n}])$ by deleting all the edges that has the two corresponding random variables separated by distance less than $\frac{b\log n}{n}$.

%First, let us try to understand the threshold for isolated nodes in the RAG. 
Next we will show that if $a-b < \pi$ then there exists an isolated vertex with high probability. It would be easier to think of each vertex as a uniform random point in $[0,2\pi]$ and the distance  between them being the Lee distance.
Define an indicator variable $A_{u}$ for every node $u$ which is 1 when node $u$ is isolated and $0$ otherwise. We have,
$$\Pr(A_{u}=1)=\bigg(1-\frac{2(a-b)\log n}{2\pi n}\bigg)^{n-1}.$$ 
Define $A=\sum_{u} A_{u}$, and hence
$$\avg[A]=n\Big(1-\frac{2(a-b)\log n}{2\pi n} \Big)^{n-1}= n^{1-\frac{(a-b)}{\pi}-o(1)}.$$ Therefore, when $a-b < \pi$, $\avg[A]=\Omega(1)$. To prove this statement with high probability we can show that the variance of $A$ is bounded. Since $A$ is a sum of indicator random variables, we have that 
$${\rm Var}(A) \le \avg[A]+\sum_{u \neq v} {\rm Cov}(A_u,A_v)=\avg[A]+\sum_{u \neq v} (\Pr(A_u=1 \cap A_v=1)-\Pr(A_u=1)\Pr(A_v=1)).$$ 
Now, consider the scenario when the  vertices $u$ and $v$ are at a distance more than $\frac{2a \log n}{n}$ apart (happens with probability $1-\frac{4a\log n}{n})$. Then the region in $[0,2\pi]$ that is between  distances $\frac{b \log n}{n}$ and $\frac{a\log n}{n}$ from both of the vertices is empty and therefore $\Pr(A_u=1 \cap A_v=1) =  
\Big(1- \frac{4(a-b) \log n}{2\pi n}\Big)^{n-2}.$
%\Pr(A_u=1)\Pr(A_v=1) = (\Pr(A_u=1))^2$.  
When the vertices  are within distance $\frac{2a \log n}{n}$ of one another, then
$
\Pr(A_u=1 \cap A_v=1) \le \Pr(A_u=1).
$
Therefore,
\begin{align*}
\Pr(A_u=1 \cap A_v=1) \le &(1-\frac{4a\log n}{2\pi n}) \Big(1- \frac{4(a-b) \log n}{2\pi n}\Big)^{n-2} + \frac{4a\log n}{2\pi n}\Pr(A_u=1)\\ 
&\le  (1-\frac{4a\log n}{2\pi n}) n^{-2(a-b)/\pi+o(1)}+ \frac{4a\log n}{2\pi n} n^{-(a-b)/\pi+o(1)}.
\end{align*}
Consequently for large enough $n$,
\begin{align*}
\Pr(A_u=1 \cap A_v=1)-\Pr(A_u=1)\Pr(A_v=1) &\le (1-\frac{4a\log n}{2\pi n}) n^{-2(a-b)/\pi+o(1)} \\+ \frac{4a\log n}{2\pi n} n^{-(a-b)/\pi+o(1)}  -& n^{-2(a-b)/\pi +o(1)} 
\le  \frac{8a\log n}{2\pi n}\Pr(A_u=1).
\end{align*}
Now,
$$
{\rm Var}(A) \le \avg[A] + \binom{n}{2}\frac{8a\log n}{2\pi n}\Pr(A_u=1) \le \avg[A](1+ 2a/\pi \log n).
$$
By using Chebyshev bound, with probability at least $1-\frac{1}{\log n}$, 
%we can upper bound the probability $\Pr(A_u=1 \cap A_v=1)$ by taking the regions of interest to be the same. Hence
%$$ \Pr(A_i=1 \cap A_j=1) \le \frac{4a \log n}{n}n^{-2(a-b)}+\bigg(1-\frac{4a \log n}{n}\bigg)n^{-4(a-b)}$$ and since $\Pr(A_i=1)\Pr(A_j=1)=n^{-4(a-b)}$, we have that
%$$ {\rm Var}(A) < n^{1-2(a-b)}+\frac{n^{2}}{2}\frac{4a \log n}{n}(n^{-2(a-b)}-n^{-4(a-b)})$$  
%Simplifying, we have that ${\rm Var}(A) < n^{1-2(a-b)}(1+2a\log n)$ which gives us using Chebychev that
$$A >n^{1-(a-b)/\pi}-\sqrt{n^{1-(a-b)/\pi}(1+2a/\pi\log n)\log n},$$
which imply for $a-b <\pi$ there will exist isolated nodes with high probability.
 %with probability $1-\frac{1}{\lambda^{2}}$.
% The second condition stems from the fact that the RAG $G(n,[r_s,r_d])$ is disconnected when $a<1$ irrespective of the value of $b$. This is because the connectivity threshold for a Random Geometric Graph $G(n,r)$ where $r=\frac{a \log n}{n}$ is $a=1$. Therefore the RGG is disconnected when $a < 1$ and if we consider the corresponding RAG, the parameter $b$ is only going to reduce the edges. Hence the RAG $G(n,[\frac{b \log n}{n},\frac{a \log n}{n}])$ cannot be connected when $a <1$ and thus we have the statement of the theorem.    
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%Now we are ready to prove the final upper bound. Note that to prove Proposition~\ref{}, we defined two events and shown that the events happen with high probability. The second event happens with high probability as long as $a >b >0$, by choosing $k$ and $\epsilon$ appropriately (that is $k = \lceil b/(a-b)\rceil+1$ and $\epsilon < \frac1{2k}$). On the other hand for the first event to happen with high probability, we needed $a-b> 1$. In the next lemma we will show that the first event happens with  

\section{The Geometric Block Model: Proof of  Theorem \ref{gbm:lower} and ~\ref{gbm:upper}}
\label{sec:gbm}

\subsection{Immediate consequence of RAG connectivity}
The following lower bound for GBM can be obtained as a  consequence of Theorem~\ref{thm:lower_bound}.

\begin{theorem}[Impossibility in GBM]\label{gbm:lowergbm}
Any algorithm to recover the partition in ${\rm GBM}(\frac{a \log n}{n},\frac{b \log n}{n})$ will give incorrect output with probability $1-o(1)$ if $a-b < \pi$ or $a < 2\pi$.
\end{theorem}
\begin{proof}
%\textcolor{red}{This part should be corrected, may be by adding the multi component proof in the appendix} 
%Recall that an edge between $2$ nodes $u$ and $v$ in the $2$-cluster GBM was formed if the associated random variables $X_u$ and $X_v$ uniformly chosen from $[0,1]$ are close in Lee distance. 

Consider the scenario that not only the geometric block model graph  ${\rm GBM}(\frac{a \log n}{n},\frac{b \log n}{n})$ was provided to us, but also the random values $X_u \in [0,2\pi]$ for all vertex $u$ in the graph were provided. We will show that we will still not be able to recover the correct partition of the vertex set $V$ with probability at least $0.5$ (with respect to choices of $X_uu, v\in V$ and any randomness in the algorithm).

In this situation, the edge $(u,v)$ where $d_L(X_u,X_v) \le \frac{b \log n}{n}$ does not give any new information than $X_u,X_v$. However the edges $(u,v)$ where $\frac{b \log n}{n} \le d_L(X_u,X_v) \le \frac{a \log n}{n}$ are informative, as existence of such an edge will imply that $u$ and $v$ are in the same part. These edges constitute a random annulus graph ${\rm RAG}(n, [\frac{b \log n}{n},\frac{a \log n}{n}])$. But if there are more than two components in this random annulus graph, then it is impossible to separate out the vertices into the correct two parts, as the connected components can be assigned to any of the two parts and the RAG along with the location values ($X_u, u \in V$) will still be consistent. 

What remains to be seen that ${\rm RAG}(n, [\frac{b \log n}{n},\frac{a \log n}{n}])$ will have $\omega(1)$ components with high probability  if $a-b < \pi $ or $a < 2\pi$. This is certainly true when $a-b < \pi$ as we have seen in Theorem~\ref{thm:lower_bound}, there can indeed be $\omega(1)$ isolated nodes with high probability. On the other hand, when $a<2\pi$, just by using an analogous argument it is possible to show that there are $\omega(1)$ vertices that do not have any neighbors on the left direction (counterclockwise). We delegate the proof of this claim as Lemma \ref{lem:disc} in the appendix.  %\textcolor{red}{Give  this proof in  appendix?} 
If there are $k$ such vertices, there must be at least $k-1$ disjoint candidates.This completes the proof.
\end{proof}

%\textcolor{red}{Fill up the corollary below} 



\begin{theorem}[GBM with known vertex locations]\label{thm:gbmplus}
Suppose a geometric block model graph ${\rm GBM}(\frac{a \log n}{n},\frac{b \log n}{n})$ is provided along with the associated  values of the locations $X_u$ for every vertex $u$. Any algorithm to recover the partition in ${\rm GBM}(\frac{a \log n}{n},\frac{b \log n}{n})$ will give incorrect output with probability $1-o(1)$ if $a-b < \pi$ or $a < 2\pi$. On the other hand it is possible to recover the partition exactly with probability $1-o(1)$ when $a-b > \pi$ and $a > 2\pi$.
\end{theorem}
\begin{proof}
We need to only prove that  it is possible to recover the partition exactly with probability $1-o(1)$ when $a-b > \pi$ and $a > 2\pi$, since the other part is immediate from Theorem~\ref{gbm:lower}. For any pair of vertices $u,v$, we can verify if $d(u,v) \in [\frac{b \log n}{n},\frac{a \log n}{n}]$. If that is the case then by just checking in the GBM graph whether they are connected by an edge or not we can decide whether they belong to the same cluster or not respectively. What remains to be shown that  all vertices can be covered by this procedure. However that will certainly be the case since ${\rm RAG}(n , [\frac{b \log n}{n},\frac{a \log n}{n}])$ is connected with high probability.
\end{proof}

Next we provide the main algorithm for recovery in GBM and its analysis.
\subsection{A motif-counting algorithm for GBM}

Suppose we are given a graph $G=(V:|V|=n,E)$ with $2$ disjoint parts, $V_1, V_2 \subseteq V$ generated according to ${\rm GBM}(r_s, r_d)$. We here provide a recovery algorithm to identify the partition, $V_1$ and $V_2$. This recovery (or clustering)  algorithm is based on counting motifs, where a motif is simply
defined as a configuration of triplets in the graph. Let us explain this principle by one particular motif,
a triangle. For any two vertices $u$ and $v$ in $V$ , where $(u, v)$ is an edge, we count the total number of
common neighbors of $u$ and $v$.


%We can observe that a pair of nodes have a very high or very low motif-count when they belong to the same cluster.  The main intuition behind our algorithm is to look at pair of nodes to label the intra-cluster edges which are easily identifiable. This procedure of identifying intra-cluster edges helps obtain the clusters whenever the graph formed by these easily identifiable edges is connected.

 The pseudocode of the algorithm is described in Algorithm ~\ref{alg:alg1}. The algorithm goes over  all edges  $(u,v)\in E$. It counts the number of triangles  containing the edge  $(u,v)$ by calling the \texttt{process} function that  %to decide if it can confidently label the pair to belong to same cluster.   The \texttt{process} function 
 counts the number of common neighbors of $u$ and $v$. % to make the decision.
   \texttt{process} outputs `true' if it is confident that the nodes $u$ and $v$ belong to the same cluster and `false' otherwise. More precisely, if the count is within some prescribed values $E_S$ and $E_D$, it returns `false'\footnote{Note that, the thresholds $E_S$ and $E_D$ refer to the maximum and minimum value of triangle-count for an `inter cluster' edge.}.The algorithm removes the edge on getting a `false' from \texttt{process} function. After processing all the edges of the network, the algorithm is left with a reduced graphs (with certain edges deleted from the original). It then finds the connected components in the graph and returns them  as the parts $V_1$ and $V_2$. %The nodes belonging to the same connected component are returned as belonging to the same cluster.



 \begin{remark}
The algorithm can iteratively maintain the connected components over the processed edges (the pairs for which process function has been called and it returned true) like the union-find algorithm. This reduces the number of queries as the algorithm does not need to  call the \texttt{process} function for the edges which are present in the same connected component. 
 \end{remark}
   

%\noindent\begin{minipage}{.5\textwidth}
%\setlength{\textfloatsep}{5pt}% Remove \textfloatsep
%\begin{algorithm}[htbp]
\captionof{algorithm}{Cluster recovery in GBM}
\begin{algorithmic}[1]\label{alg:alg1}
{
\REQUIRE GBM $G = (V,E)$, $r_s, r_d$
\FOR {$(u,v)\in E$}
\IF{{\rm process}($u,v,r_s,r_d$)}
\STATE continue
\ELSE
\STATE $E.remove((u,v))$
\ENDIF
\ENDFOR
\RETURN {\rm connectedComponent}$(V,E)$
}
\end{algorithmic}
%\end{algorithm}
%\end{minipage}
 
\captionof{algorithm}{\texttt{process}}
\begin{algorithmic}[1]\label{alg:process}
{
\REQUIRE $u$,$v$, $r_s$, $r_d$
\ENSURE  true/false\\
\COMMENT{Comment: $t_1=\min\{t: (\frac{b}{\pi}+t)\log \frac{b+\pi t}{b}-t > 1\}, t_2=\min\{t : (\frac{b}{\pi}-t)\log \frac{b-\pi t}{b}+t > 1$ and $E_S  = (\frac{b}{\pi} +t_1)\frac{\log n}{n}$ and $E_D  = (\frac{b}{\pi} - t_2)\frac{\log n}{n}$}
\STATE count $\leftarrow |\{z: (z,u)\in E, (z,v)\in E\}|$
\IF{$\frac{\text{count}}{n} \ge E_S(r_d,r_s)$ or $\frac{\text{count}}{n} \le E_D(r_d,r_s)$}
\RETURN true
\ENDIF
\RETURN false
}
\end{algorithmic}
%\end{minipage}


%Next, we describe 
%The \texttt{process} function counts the number of common neighbors of two nodes and then compares the difference of the count with
%two functions of $r_d$ and $r_s$, called $E_D$ and $E_S$. 

The crucial difference of this algorithm from the previously proposed motif-based algorithm in \citep{galhotra2017geometric} is the following. The algorithm of  \citep{galhotra2017geometric} used a \texttt{process} function that compared difference of the triangle-count from $E_D$ and $E_S$, and based on that would assign vertices to either of the two parts. In this paper, the \texttt{process} function checks whether the count of triangles is between $E_S$ and $E_D$, and the algorithm just removes the edge from the  graph if it is. We show that this leads to much improvement in performance.


The distribution of the number of common neighbors given $(u,v)\in E$ and $d(u,v)=x$ is given in Table ~\ref{tab:tab1}. %We  provide the values of  $E_D$ and $E_S$  in Theorem \ref{th:main} for the regime of $r_s> 4r_d$.}  
As throughout this paper, we have assumed that there are only two clusters of equal size. The functions change when the cluster sizes are different. %Our analysis described in later sections can be used to calculate new function values.
 In the table, $u\sim v$ means $u$ and $v$ are in the same cluster. 
%Similarly, the \texttt{process} function can be run on other set of motifs by fixing two nodes. On considering a larger set of motifs, the \texttt{process} function can take a majority vote over the decisions received from different motifs.

\begin{table*}[htbp]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|p{3.2cm}|p{3cm}|p{3cm}|p{3.6cm}|} 
 \hline
$(u,v) \in E$ & \multicolumn{2}{c}{Distribution of count ($r_s>2r_d$)}&    \multicolumn{2}{c|}{Distribution of count ($r_s\le 2r_d$)} \\
 $d(u,v) =x$      & $u \sim v,  x\leq r_s$ & $u \nsim v, x\leq r_d$ &  $u \sim v, x\leq r_s$ & $u \nsim v, x\leq r_d$\\
 \hline
Motif : $z\mid (z,u)\in E, (z,v)\in E$   &  {\correct{${\rm Bin}(\frac{n}{2}-2,\frac{2r_s-x}{2\pi})+\mathbb{1}\{x\leq 2r_d\}{\rm Bin}(\frac{n}{2},\frac{2r_d-x}{2\pi})$}} & ${\rm Bin}(n-2,\frac{r_{d}}{\pi})$ &  {\correct{${\rm Bin}(\frac{n}{2}-2,\frac{2r_s-x}{2\pi})+{\rm Bin}(\frac{n}{2},\frac{2r_d-x}{2\pi})$}}  & \correct{${\rm Bin}(n-2, \frac{\min(r_{s}+r_d-x,2r_d)}{2\pi})$}\\
% \hline
%Motif 2: $z\mid (z,u)\in E, (z,v)\notin E$ & {\correct{${\rm Bin}(\frac{n}{2}-2,x)+{\rm Bin}(\frac{n}{2},\min(x,2r_d))$ }}& \correct{${\rm Bin}(\frac{n}{2}-1,2(r_{s}-r_{d}))  $ }& \correct{${\rm Bin}(n-2, x)$} & \correct{${\rm Bin}(\frac{n}{2}-1,r_s-r_d+x + \max(r_s-x-r_d,0)) + {\rm Bin}(\frac{n}{2}-1,\max(x+r_d-r_s,0)) $ }\\
% \hline
%Motif 3:  $z\mid (z,u)\notin E, (z,v)\in E$  &{\correct{${\rm Bin}(\frac{n}{2}-2,x)+{\rm Bin}(\frac{n}{2},\min(x,2r_d))$ }} & \correct{${\rm Bin}(\frac{n}{2}-1,2(r_{s}-r_{d})) $ }& \correct{${\rm Bin}(n-2, x)$} &  \correct{${\rm Bin}(\frac{n}{2}-1,r_s+r_d-x + \max(r_s-x-r_d,0)) + {\rm Bin}(\frac{n}{2}-1,\max(x+r_d-r_s,0)) $ }\\
% \hline
% Motif 4: $z\mid (z,u)\notin E, (z,v)\notin E$  &{\correct{${\rm Bin}(\frac{n}{2}-2,1-(x+2r_s))+\mathbb{1}\{x \le 2r_d\}{\rm Bin}(\frac{n}{2},1-(x+2r_d))+\mathbb{1}\{x > 2r_d\}{\rm Bin}(\frac{n}{2},1-4r_d) $}} & \correct{${\rm Bin}(n-2,1-2r_s) $ }& \correct{${\rm Bin}(\frac{n}{2}-2,1-(x+2r_s))+{\rm Bin}(\frac{n}{2},1-(x+2r_d))$ } &  \correct{$\mathbb{1}\{x \le r_s-r_d\}{\rm Bin}(n-2,1-2r_s)+\mathbb{1}\{x >r_s-r_d\}{\rm Bin}(n-2,1-(x+r_s+r_d))$ }\\
\hline
\end{tabular}}
\end{center}
\caption{Distribution of motif count for an edge $(u,v)$ conditioned on the distance between them $d(u,v) = d_L(X_u, X_v) = x$, when there are two equal sized clusters. Here ${\rm Bin}(n,p)$ denotes a binomial random variable with mean $np$.\label{tab:tab1}}
\end{table*}
 
 
 
 
%considering different values of $r_s$ and $r_d$,

% 2 & $B+B$ & $B$ & $-\frac{(3r_{s}-2r_{d})(r_{s}-2r_{d})}{4r_{s}}$ $< 0$ &
% $B(n,r_{s}/2)$ & $B(n,\frac{(r_{s}-r_{d})^{2}}{r_{d}}+\frac{(2r_{d}-r_{s})(3r_{s}-2r_{d})}{4r_{d}}+\frac{(2r_{d}-r_{s})^{2}}{4r_{d}})$ =
% $B(n,\frac{r_{s}^{2}+2r_{d}^{2}-2r_{s}r_{d}}{r_{d}} )$& $\frac{(r_{s}-r_{d})(2r_{d}-r_{s})}{2r_{d}} > 0$ \\
%\hline
% 3 $z\mid $$(z,u)\notin E$, $(z,v)\in E$ & $B(\frac{n}{2},r_{s}/2)+B(\frac{n}{2},\frac{2r_{d}(r_{s}-r_{d}}{r_{s}})$ & $B(n,r_{s}-r_{d})$ & $-\frac{(3r_{s}-2r_{d})(r_{s}-2r_{d})}{4r_{s}}$ $< 0$ &
% $B(n,r_{s}/2)$ & $B(n,\frac{(r_{s}-r_{d})^{2}}{r_{d}}+\frac{(2r_{d}-r_{s})(3r_{s}-2r_{d})}{4r_{d}}+\frac{(2r_{d}-r_{s})^{2}}{4r_{d}})$ =
% $B(n,\frac{r_{s}^{2}+2r_{d}^{2}-2r_{s}r_{d}}{r_{d}} )$& $\frac{(r_{s}-r_{d})(2r_{d}-r_{s})}{2r_{d}} > 0$ \\
%\hline
 
 
   % Note that, our algorithm counts motifs only for edges, and does not count motifs for more than $n-1$ edges, as there are only $n$ vertices to be be assigned to clusters.
% \begin{remark}
%If we are given k clusters ($k>2$), our analysis can be extended to calculate new values of $E_S$ and $E_D$. If there exists a palpable gap between the two values, we can extend the Algorithm \ref{alg:alg1} to  identify the true assignment of each node.
% \end{remark}
   
\subsection{Analysis of Algorithm~\ref{alg:alg1}}
~\label{sec:theory}
The critical observation made in \citep{galhotra2017geometric} was the fact that given a GBM graph $G(V,E)$ with two clusters $V = V_1 \sqcup V_2$, and  a pair of vertices $u,v \in V$, the events $\cE^{u,v}_z, z \in V$ of any other vertex $z$ being a common neighbor of 
both $u$ and $v$ given $(u,v) \in E$ are dependent ; however given the distance between the corresponding random variables  \correct{$d_L(X_u,X_v) =x$}, the events %$\cE^{u,v}_z , z \in V \mid d_L(X_u,X_v) =x$ 
are independent. %\correct{It is important to note that the event $\cE^{u,v}_z, z \in V$ is independent conditional on the distance between $u$ and $v$ (even when $(u,v)\notin E$). The independence does not exist if we assume only the presence of edge between $u$ and $v$. } 
Moreover, the probabilities of $\cE^{u,v}_z\mid (u,v) \in E$ are different when $u$ and $v$ are in the same cluster and when they are in different clusters. Therefore the count of the common neighbors are going to be different, and substantially separated with high probability %(due to being sums of independent random variables)
 for two vertices in cases when they are from the same cluster or from different clusters. %This will lead the function \texttt{process} to correctly characterize two vertices as being from same or different clusters with high probability.  

We quote here the following two lemmas for a ${\rm GBM}(r_s,r_d)$ graph $G(V,E)$, that appeared in \citep{galhotra2017geometric}. %with two equal-sized (unknown) clusters $V = V_1 \sqcup V_2$, and parameters $r_s,r_d$.





\begin{lemma}\label{lem:sep}
For any two vertices $u,v \in V_i: (u,v) \in E, i =1,2$ such that $d_L(X_u,X_v) = x$ belonging to the same cluster, the count of common neighbors $C_{u,v} \equiv |\{z\in V: (z,u), (z,v) \in E\}|$ is a random variable distributed according to ${\rm Bin}(\frac{n}{2}-2, \frac{2r_s-x}{2\pi})$ when $r_s \geq x> 2r_d$ and according to ${\rm Bin}(\frac{n}{2}-2,\frac{2r_s-x}{2\pi})+{\rm Bin}(\frac{n}{2},\frac{2r_d-x}{2\pi})$ when $x \leq min(2r_d,r_s)$, where ${\rm Bin}(n,p)$ is a binomial random variable with mean $np$.
\end{lemma}
\begin{lemma}\label{lem:sep2}
For any two vertices $u\in V_1,v \in V_2: (u,v) \in E$ such that $d_L(X_u,X_v) = x$ belonging to different clusters, the count of common neighbors $C_{u,v} \equiv |\{z\in V: (z,u), (z,v) \in E\}|$ is a random variable distributed according to ${\rm Bin}(n-2,\frac{2r_{d}}{2\pi})$ when $r_s > 2r_d$ and according to ${\rm Bin}(n-2,\frac{min(r_{s} + r_d -x,2r_d)}{2\pi})$ when $r_s \leq 2r_d$ and $x\leq r_d$.
\end{lemma}
%Similar lemmas exists for other motifs as well. We describe those in detail in the appendix. Here let us give the proof of Lemma \ref{lem:sep}. The proof of Lemma \ref{lem:sep2} will follow similarly. These expressions can also be generalized straightforwardly when the clusters are of unequal sizes, but we omit those for clarity of exposition. 

Since the proofs have already appeared in \citep{galhotra2017geometric}, we just give proof of Lemma \ref{lem:sep} for completeness.

\begin{proof}[Proof of Lemma \ref{lem:sep}]
%Let $X_w\in [0,1]$ be the uniform random variable associated with $w \in V$. Let us also denote by $\dist(X,Y) \equiv \min\{|X - Y|, 1- |X- Y|\}, X,Y \in \reals$. 
Without loss of generality, assume $u,v \in V_1$. For any vertex $z \in V$, let $\cE^{u,v}_z \equiv \{(u,z), (v,z) \in E\}$ be the event that $z$ is a common neighbor.
For $z\in V_1$,
\begin{align*}
&\Pr(\cE^{u,v}_z) =\Pr( (z,u) \in E, (z,v) \in E \mid \dist(X_u,X_v) =x) \\
& = \frac{2r_s - x}{2\pi} .
\end{align*}
For $z \in V_2$, we have, 
\begin{align*}
&\Pr(\cE^{u,v}_z) =  \Pr( (z,u), (z,v) \in E \mid \dist(X_u,X_v) =x) \\
& =  \begin{cases}\frac{2r_d-x}{2\pi} & \text{ if } x<2r_d \\ 0 & \text{ otherwise} \end{cases} .
\end{align*}
Now since there are $\frac{n}2-2$ points in $V_1 \setminus \{u,v\}$ and $\frac{n}2$ points in $V_2$, we have the statement of the lemma. 
\end{proof}
%The proof of Lemma \ref{lem:sep2} is similar and we delegate it to the appendix in the supplementary material.

%By leveraging the concentration of binomial random variables, in our algorithm we just check whether the count of common neighbors is closer to the average value of the random variable described in Lemma \ref{lem:sep} or in Lemma \ref{lem:sep2}. While more general statements are possible, we give a theorem concentrating on the special case when $r_s, r_d \sim \frac{\log n}{n}$.
 

At this point note  that, in a ${\rm GBM}(r_s,r_d)$ for any edge $u,v$ that do not belong to the same part, the expected total number of common neighbors of  $u$ and $v$ does not depend on  their distance. We will next show that in this case the normalized total number of common neighbors is concentrated around $2r_d$. Therefore, when Algorithm~\ref{alg:alg1} finished removing all the edges, with high probability all the `inter-cluster' edges are removed. However, some of the `in-cluster' edges will also be removed in the process. This is similar to the case when from an ${\rm RGG}(n, r_s)$, all the edges that correspond to a distance close to $2r_d$ has been removed. 
This situation is shown for the case when $r_s \ge 2r_d$ in Figure~\ref{fig:gbm}.
Finally we show that the edge-reduced  ${\rm RGG}(n, r_s)$ is still connected under certain condition. In  what follows we will assume the ${\rm GBM}(r_s,r_d)$ with $r_s\ge 2r_d$. We point out that the other case can also be analyzed in the similar way.

In the next lemma, we just show concentration  of the count made in \texttt{process}.

\begin{figure}
\centering
\begin{tikzpicture}
%\draw[help lines, color=gray!30, dashed] (-1,-1) grid (2,2);

%\draw[fill=gray]  (2,1) -- (4,3) -- (4,0) -- (2,0) -- cycle;
%\draw[->,ultra thick] (-0.5,0)--(4,0) node[right]{$a$};
%\draw[->,ultra thick] (0,-0.5)--(0,4) node[above]{$b$};

\draw[->] (0,0)--(5,0); 
\draw[->] (0,0)--(0,5); 
\draw[blue, ultra thick] (0,4.2)--(2.4,1.8); 
\draw[blue, ultra thick] (2.4,1.8)--(3,1.5); 
\draw[red, ultra thick, dashed] (0,2.4)--(1.2,2.4); 
\draw[gray,<->] (0,-0.5)--(1.2,-0.5); 
\draw[gray,<->] (1.2,-0.5)--(2.4,-0.5); 
\draw[blue!50, <->] (0,-0.7)--(3,-0.7); 
\draw[red,<->] (-0.5,0)--(-0.5,1.2); 
\draw[red,<->] (-0.5,1.2)--(-0.5,2.4); 
\draw[violet,<->] (-1,0)--(-1,3); 
\draw[red,<->] (-1,3)--(-1,4.2); 
\draw[red,<->] (-1.5,3)--(-1.5,1.8); 
\draw (1.2,0.1)--(1.2,-0.1)node at (1.2,-0.25) {$r_d$}; 
\draw (2.4,0.1)--(2.4,-0.1)node at (2.4,-0.25){$2r_d$}; 
\draw (3,0.1)--(3,-0.1)node at (3,-0.25){$r_s$}; 
\draw[gray,dashed] (3,0)--(3,1.5); 
\draw[gray,dashed] (1.2,0)--(1.2,2.4); 
\draw[gray,dashed] (2.4,0)--(2.4,1.8); 

\draw[gray,dashed] (-1.5,1.8)--(2.4,1.8); 
\draw[gray,dashed] (-1,3)--(1.2,3); 
\node at (-0.3,2.6){$\frac{r_d}{\pi}$}; 
\node at (5,-0.2){$x$}; 
\draw (0.1,4.2)--(-0.1,4.2);
\node at (-0.7,4.4){$\frac{r_s+r_d}{2\pi}$}; 
\draw[<->, gray ] (3,5)--(3.5,5)node at (3.8,5) {${r_d}$}; 
\draw[<->, blue!50 ] (3,4.5)--(3.5,4.5)node at (3.8,4.5) {${r_s}$}; 

\draw[<->, red ] (3,3.5)--(3.5,3.5)node at (3.8,3.5) {$\frac{r_d}{2\pi}$}; 
\draw[<->, violet ] (3,4)--(3.5,4)node at (3.8,4) {$\frac{r_s}{2\pi}$}; 
\draw[blue, ultra thick ] (3,3)--(3.5,3)node at (7.5,3) {Intra-cluster edge: $ \begin{cases}
\frac{r_s+r_d-x}{2\pi}, x\leq 2r_d\\
\frac{r_s-x/2}{2\pi}, 2r_d< x\le r_s
\end{cases}$}; 
\draw[red, ultra thick, dashed ] (3,2)--(3.5,2)node at (6.5,2) {Inter-cluster edge: $\frac{r_d}{\pi}, 0\le x\le r_d$}; 
%\node[below] at (1,0) {$1$};
%\node[below] at (0.5,0) {$0.5$};
%\node[left] at (0,0.5) {$0.5$};
%\draw [blue, ultra thick]  (9,1)--(10.08,1.04)--(10.5,1.25) -- (11,1.5) -- (13,2) -- (15,2.5)  -- (16,3);% -- cycle;

%\draw[fill=gray,transparent]  (1,0.5) -- (4,3) -- (4,0) -- (1,0) -- cycle;
\end{tikzpicture}
\caption{Average number of common neighbors of $(u,v) \in E$  for varying values of $d(u,v) =x$ when $r_s\ge2r_d$.\label{fig:gbm}}
\end{figure}

\begin{lemma}\label{lem:defn}
Suppose we are given the graph $G(V,E)$ generated according to ${\rm GBM}(r_s\equiv \frac{a\log n}{n},r_d\equiv \frac{b\log n}{n}); a \ge 2b.$ 
Our algorithm with $E_S = (\frac{b}{\pi} + t_1)\frac{\log n}{n}$ and $E_D = (\frac{b}{\pi} - t_2)\frac{\log n}{n}$, removes
all the edges $(u,v)\in E$ such that   $u$ and $v$ are in different parts with probability at least $1-o(1)$, where
%For any pair of nodes $(u,v)\equiv e\in E,$ such that   $u$ and $v$ are in different parts, our algorithm with $E_S = (2b + t_1)\frac{\log n}{n}$ and $E_D = (2b - t_2)\frac{\log n}{n}$, removes the edge $e$ with a probability of at least $1-O\left(\frac{1}{n\log^2 n}\right)$ where
\begin{align*}
t_1&=\min\{t: (\frac{b}{\pi}+t)\log \frac{b+\pi t}{b}-t > 1\} \\
t_2&=\min\{t : (\frac{b}{\pi}-t)\log \frac{b-\pi t}{b}+t > 1\}.
\end{align*}
\end{lemma} 

\begin{proof}
Let $Z$ denote the random variable that equals the number of common neighbors of two nodes $u,v \in V: (u,v) \in E$ such that $u,v$ are from different parts of the GBM. Using Lemma \ref{lem:sep2}, we know that $Z$ is sampled from the distribution ${\rm Bin}(n-2,\frac{2r_d}{2\pi})$, where $r_d = \frac{b\log n}{n}$. Therefore,
\begin{align*}
\Pr(Z \ge nE_S) \le \sum_{i=nE_S}^{n} {n \choose i}(\frac{r_d}{\pi})^{i}(\frac{\pi-r_d}{\pi})^{n-i} \le \exp\Big(-nD\Big((\frac{b}{\pi} + t_1)\frac{\log n}{n}\|\frac{b\log n}{\pi n}\Big)\Big),
\end{align*}
where $D(p\|q)\equiv p\log\frac{p}{q}+ (1-p)\log \frac{1-p}{1-q}$ is the KL divergence between Bernoulli($p$) and Bernoulli($q$) distributions.
%We will use the following approximation for the Divergence
It is easy to see that,
\begin{align*}
nD(\frac{\alpha \log n}{n}||\frac{\beta \log n}{n})= \Big(\alpha\log\frac{\alpha}{\beta}+(\alpha-\beta)\Big)\log n-o(\log n).
\end{align*}
Therefore $\Pr(Z \ge nE_S) \le \frac{1}{n(\log n)^2}$ because 
$
(\frac{b}{\pi}+t_1)\log\frac{b+\pi t_1}{b}-t_1 > 1.
$
Similarly, we have that 
\begin{align*}
\Pr(Z \le nE_D) \le \sum_{i=0}^{nE_D} {n \choose i}(\frac{r_d}{\pi})^{i}(\frac{\pi-r_d}{\pi})^{n-i} \le \exp(-nD((\frac{b}{\pi}-t)\frac{\log n}{n}\|\frac{b\log n}{\pi n}))\le \frac{1}{n(\log n)^2}.
\end{align*}
%and there we must have that $\Pr(Z \le E_D) \le o(\frac{1}{n\log n})$ if
%\begin{align*}
%(2b-t)\log \frac{2b-t}{2b}+t > 1
%\end{align*}
So all of the edges will be removed by Algorithm~\ref{alg:alg1}   with probability $1 - O(\frac{n \log n}{n(\log n)^2}) =1 -o(1)$, as with probability $1-o(1)$ the total number of edges in the graph is $O(n \log n)$.
\end{proof}
 
After Algorithm~\ref{alg:alg1}  finishes, in the edge-reduced ${\rm GBM}(\frac{a\log n}{n},\frac{b\log n}{n})$, all the edges are `in-cluster' edges with high probability. However some of the  
`in-cluster' edges are also deleted, namely, those that has a count of common neighbors between $E_S$ and $E_D$. In the next two lemmas, we show the necessary condition on  the `in-cluster' edges such that they do not get removed by Algorithm~\ref{alg:alg1}.  



\begin{lemma}
Suppose we have the graph $G(V,E)$ generated according to ${\rm GBM}(r_s \equiv \frac{a\log n}{n},r_d\equiv \frac{b\log n}{n}), a \ge 2b$. Define $t_1,t_2, E_D,E_S$ as in  Lemma~\ref{lem:defn}. Consider an edge $(u,v) \in E$ where $u,v$ belong to the same part of the GBM and let  $d(u,v)\equiv x \equiv \frac{\theta \log n}{n}$. Suppose $\theta$ satisfies {\bf either} of the following conditions:
\begin{enumerate}
\item $
\frac{1}{2}\Big( (\frac{2b}{\pi}+2t_1)\log \frac{4b+4\pi t_1}{2a-\theta}+\frac{2a-\theta}{2\pi}-(\frac{2b}{\pi}+2t_1)\Big) > 1 \quad \text{ and } \frac{2a-\theta}{2\pi} \ge \frac{2b}{\pi}+2t_1
$
\item $
\frac{1}{2}\Big(\frac{2b}{\pi}-2t_2)\log \frac{4b-4\pi t_2}{2a-\theta}+\frac{2a-\theta}{2\pi}-(\frac{2b}{\pi}-2t_2)\Big) > 1
\quad \text{and} \quad 
a \ge \theta \ge \max\{2b,2a-4b+4\pi t_2\}.
$
\end{enumerate}
Then Algorithm~\ref{alg:alg1} with $E_S  = (\frac{b}{\pi_1} +t_1)\frac{\log n}{n}$ and $E_D  = (\frac{b}{\pi} - t_2)\frac{\log n}{n}$ will not remove this edge with probability at least $1- O(\frac1{n (\log n)^2})$.
%
%Given a pair of nodes $e=(u,v)\in E$ such that $u,v\in C_1$, connected by an edge, our algorithm does not remove the edge $e$ on considering the threshold $E_S  = (2b +t_1)\frac{\log n}{n}$  alone
%when $\dist{(X_u,X_v)} = x = \frac{\theta \log n}{n}$(say) satisfies the following:
%
\label{lem:esed}
\end{lemma}
\begin{proof}
Let $Z$ be the number of common neighbors of $u,v$. % \in V: u \sim v,(u,v) \in E, \dist(X_u,X_v) = x$
%. Let us also denote $\mu_s(x)= \avg(Z|u \sim v, \dist(X_u,X_v)=x)$, 
Recall that, $u$ and $v$ are in the same cluster. 
We know from Lemma \ref{lem:sep2} that $Z$ is sampled from the distribution ${\rm Bin}(\frac{n}{2}-2,\frac{2r_s-x}{2\pi})+{\rm Bin}(\frac{n}{2},\frac{2r_d-x}{2\pi})$ when $x \le 2r_d$, and from the distribution ${\rm Bin}(\frac{n}{2}-2,\frac{2r_s-x}{2\pi})$ when $x \ge 2r_d$. 
%Notice that we remove an edge if the motif count for that edge is less than $nE_S$ (assuming that there is only a single threshold). Therefore, 
We have,
\begin{align*}
&\Pr(Z \le nE_S)\\
&=
\begin{cases}
\sum_{i=0}^{nE_S}{\frac{n}{2}-2 \choose i} (\frac{2r_s-x}{2\pi})^{i}(\frac{2\pi-2r_s+x}{2\pi})^{\frac{n}{2}-i-2}\sum_{j=0}^{nE_S-i}{\frac{n}{2} \choose j} (\frac{2r_d-x}{2\pi})^{j}(\frac{2\pi-2r_d+x}{2\pi})^{\frac{n}{2}-j} \text{ if $x\le 2r_d$ }\\
\sum_{i=0}^{nE_s}{\frac{n}{2}-2 \choose i} (\frac{2r_s-x}{2\pi})^{i}(\frac{2\pi-2r_s+x}{2\pi})^{\frac{n}{2}-i} \text{ otherwise} \\
\end{cases} \\
& \le e^{-\frac{n}{2}D(2E_S|| \frac{(2a-\theta)\log n}{2\pi n})} \text{ since  } \frac{2a-\theta}{2\pi} \ge \frac{2b}{\pi}+2t_1\\
& \le e^{-\frac{n}{2}D(\frac{(2b+2\pi t_1)\log n}{\pi n}|| \frac{(2a-\theta)\log n}{2\pi n})} \le \frac{1}{n \log^2 n},
\end{align*}
because of condition 1 of this lemma. Therefore, this edge will not be deleted with high probability.
%We have upper bounded  above the second sum in the case where $x \le 2r_d$ by $1$. %because in order to bound it by a Divergence term, we would have needed $2b-\theta \le 4b+2t_1$ which is not possible. Since $4b+2t_1$ is always greater than $2b-\theta$, the best upper bound for $\sum_{j=0}^{nE_S-i}{\frac{n}{2} \choose j} (2r_d-x)^{j}(1-2r_d+x)^{\frac{n}{2}-j}$ is just $1$)\\
%Hence $\Pr(Z \le E_S)=o(\frac{1}{n \log n})$ if we have that
%\begin{align*}
%\frac{1}{2}\Big((4b+2t_1)\log \frac{4b+2t_1}{2a-\theta}+2a-\theta-4b-2t_1\Big) > 1
%\end{align*}
%\end{proof}
%
%
%
%
%
%
%\begin{lemma}
%Given a pair of nodes $e=(u,v)\in E$ such that $u,v\in C_1$, connected by an edge, our algorithm does not remove the edge $e$ on considering the threshold $E_D  = (2b - t_2)\frac{\log n}{n}$  alone
%when $\dist{(X_u,X_v)} = x = \frac{\theta \log n}{n}$(say) satisfies the following:
%
%where $t_2$ is defined in lemma \ref{lem:diffdivx}.
%\end{lemma}
%\begin{proof}
%Let $Z$ denote the random variable that equals the number of common neighbors of two nodes $u,v \in V: u \sim v,(u,v) \in E, \dist(X_u,X_v) = x$
%. Let us also denote $\mu_s(x)= \avg(Z|u \sim v, \dist(X_u,X_v)=x)$, 
%where $u\sim v$ means $u$ and $v$ are in the same cluster. 
%
%Recall that $Z$ is sampled from the distribution ${\rm Bin}(\frac{n}{2}-2,2r_s-x)+{\rm Bin}(\frac{n}{2},2r_d-x)$ when $x \le 2r_d$ and from the distribution ${\rm Bin}(\frac{n}{2}-2,2r_s-x)$ when $x \ge 2r_d$. Notice that Algorithm we remove an edge if the motif count for that edge is more than $nE_D$ (assuming that there is only a single threshold). Therefore, for $x \le 2r_d$, we have that (becuase one of the terms from the 2 distributions has to be more than $\frac{nE_D}{2}$)

Similarly, let us find the probability of $Z \ge n E_D = (\frac{b}{\pi}-t_2) \log n.$
Let us just assume the worst case when  $\theta \le 2b$: that the edge is being deleted (see condition 2, this is prohibited if that condition is satisfied).
%
% or $\theta \le 2b$, $Z$ is distributed according  to ${\rm Bin}(\frac{n}{2}-2,2r_s-x)+{\rm Bin}(\frac{n}{2},2r_d-x)$, i.e., $\avg Z = r_s+r_d- x = (a+b -\theta)\frac{\log n}{n} $
Otherwise, $\theta > 2b $ and,
%\begin{align*}
%\Pr(Z \ge nE_D) 
%
%&\le \sum_{i=\frac{nE_D}{2}}^{n}{\frac{n}{2}-2 \choose i} (2r_d-x)^{i}(1-2r_d+x)^{\frac{n}{2}-i-2}+\sum_{i=\frac{nE_D}{2}}^{n}{\frac{n}{2} \choose i} (2r_s-x)^{i}(1-2r_s+x)^{\frac{n}{2}-i}\\
%&\le e^{-\frac{n}{2}D(E_D||2r_d-x)}+e^{-\frac{n}{2}D(E_D||2r_s-x)} \text{  if    } 2a-\theta \le 2b-t_2
%\end{align*}
%But this implies that $\theta \ge 2a-2b$ which is a contradiction to the fact that $\theta \le 2b$ since we have assumed that $a\ge 2b$. Hence, we will ignore the case when $\theta \le 2b$ and only concentrate on the case when $\theta \ge 2b$. Hence, we have that
\begin{align*}
\Pr(Z \ge nE_D)&=\sum_{i=nE_D}^{n}{\frac{n}{2}-2 \choose i} (\frac{2r_s-x}{2\pi})^{i}(\frac{2\pi-2r_s+x}{2\pi})^{\frac{n}{2}-i-2} \\
&\le e^{-\frac{n}{2}D(2E_D\|\frac{(2a-\theta)\log n}{2\pi n})} \text{   if   } \frac{2a-\theta}{2\pi} \le \frac{2b}{\pi}-2t_2\\
&= e^{-\frac{n}{2}D(\frac{(2b-2\pi t_2)\log n}{\pi n}\|\frac{(2a-\theta)\log n}{2\pi n})} \le \frac{1}{n \log^2 n},
\end{align*}
because of condition 2 of this lemma.
%Hence $\Pr(Z \le nE_D)=o(\frac{1}{n \log n})$ if 
%\begin{align*}
%\frac{1}{2}\Big((4b-2t_2\log\frac{4b-2t_2}{2a-\theta}+2a-\theta-4b+2t_{2}\Big) > 1
%\end{align*} 
\end{proof}


Now we are in a position to prove our main theorem from this part. Let us restate this theorem.

\begin{theorem}[Restating of Theorem~\ref{gbm:upper}]%\label{gbm:upper}
Suppose we have the graph $G(V,E)$ generated according to ${\rm GBM}(r_s \equiv \frac{a\log n}{n},r_d\equiv \frac{b\log n}{n}), a \ge 2b$. 
Define,
\begin{align*}
t_1 &=\min\{t: (\frac{b}{\pi}+t)\log \frac{b+\pi t}{b}-t > 1\} \\
t_2 &=\min\{t : (\frac{b}{\pi}-t)\log \frac{b-\pi t}{b}+t > 1\}. \\
\theta_1 &=\max\{\theta:\frac{1}{2}\Big( (\frac{2b}{\pi}+2t_1)\log \frac{4b+4\pi t_1}{2a-\theta}+\frac{2a-\theta}{2\pi}-(\frac{2b}{\pi}+2t_1)\Big) > 1 \quad \text{ and } \frac{2a-\theta}{2\pi} \ge \frac{2b}{\pi}+2t_1\} \\
\theta_2 &=\min\{\theta:\frac{1}{2}\Big(\frac{2b}{\pi}-2t_2)\log \frac{4b-4\pi t_2}{2a-\theta}+\frac{2a-\theta}{2\pi}-(\frac{2b}{\pi}-2t_2)\Big) > 1
\quad \text{and} \quad a \ge \theta \ge \max\{2b,2a-4b+4\pi t_2\}. \\
\end{align*}

Then Algorithm~\ref{alg:alg1} with $E_S  = (\frac{b}{\pi} +t_1)\frac{\log n}{n}$ and $E_D  = (\frac{b}{\pi} - t_2)\frac{\log n}{n}$ will recover the correct partition  in the GBM with  probability $1-o(1)$  if   $a-\theta_2+\theta_1>2\pi$ OR $a-\theta_2 > 2\pi, a>4\pi$. 
\end{theorem}
\begin{proof}
From Lemma~\ref{lem:defn}, we know that after Algorithm~\ref{alg:alg1} goes over all the edges, the edges with end-points being in different parts of the GBM are all removed with probability $1-o(1)$. 
There are $O(n \log n)$ edges in the GBM with  probability $1-o(1).$
From Lemma~\ref{lem:esed}, 
we can say that no edge with both ends at the same part is deleted with probability at least $1-o(1)$ (by simply applying a union bound).

After Algorithm~\ref{alg:alg1} goes over all the edges, the remaining edges from a disjoint union of two random annulus graphs of $\frac{n}{2}$ vertices each. For any two vertices $u,v$ in the same part, there will be an edge if $d(u,v) \in [0,\theta_1] \cup [\theta_2, a]$. From Corollary \ref{cor:patch}, it is evident that each of these two parts (each part  is of size $\frac{n}{2}$) will be connected if either $a-\theta_2+\theta_1>4\pi$ or $a-\theta_2 > 2\pi, a>4\pi$.
\end{proof}
% if either of conditions 1 or 2 of this lemma is satisfied, with probability at least $1-o(1)$.

%By Lemma \ref{lem:numedge} , we know that the maximum number of edges in $GBM(\frac{a \log n}{n},\frac{b \log n}{n})$ is $O(n \log n)$. Hence with a probability of $1-o(1)$ none of the edges $(u,v) \in E \mid u \sim v, \dist(u,v)=\frac{\theta \log n}{n}$ where $\theta \le \theta_1$ or $\theta \ge \theta_2$ is not removed by Algorithm \ref{alg:process}. Additionally, observe that all intercluster edges will be removed. Hence, if we obtain 2 connected components, then we can simply output them as the $2$ clusters and hence in order to gurantee that there exists only 2 connected components, we use Lemma \ref{lem:pat} to complete the proof. 




%When $r_s>2r_d$, Algorithm \ref{alg:alg1} with $E_S = (2b + t^{\star})\frac{\log n}{n}$ and $E_D = (2b - t^{\star})\frac{\log n}{n}$ can recover the clusters $V_1, V_2$ accurately with a probability of $1 - o(1)$ if  $a-\theta_2+\theta_1>2$ or $a-\theta_2 > 1$ or
%$
%\begin{cases}
%2(a-\theta_2)+ \theta_1/2 > 2 \text{ when } a-\theta_2<\theta_1 \text{ and }\theta_2>3\theta_1/2\\
%\theta_2-\theta_1 > 2 \text{ when } a-\theta_2<\theta_1 \text{ and }\theta_2\le 3\theta_1/2\\
%a > 2 \text{ when } a-\theta_2\ge \theta_1 \text{ and } \theta_2\le 3\theta_2/2 \\
%(a-\theta_2)+ 3\theta_1/2  > 2 \text{ when } a-\theta_2\ge \theta_1 \text{ and } \theta_2>3\theta_1/2\\
%\end{cases}$
%\end{theorem}
 It is also possible to incorporate the result of Corollary \ref{cor:extra} as well to get somewhat stronger recovery guarantee for our algorithm.



%\bibliographystyle{plainnat}
%\bibliography{bibfile}

%\appendix
\subsection{Omitted proofs}
\begin{proof}[Proof of Corollary \ref{cor:extra}]
Consider a node $u$ and assume that the position of $u$ is $0$. Associate a random variable $A_u^i$ for $i \in \{1,2,3,4\}$ which takes the value of $1$ when there does not exist any node $x$ such that 

\begin{figure}[h]
\centering
\begin{tikzpicture}[thick, scale=0.9]
\draw [black,<->] (-0.5,1.8) -- (-1,1.8)node at (0.5,1.8) {$a-b-\frac{c}{2}$};;
\draw [gray,<->] (-0.5,1.3) -- (-1,1.3)node at (0.5,1.3) {$\frac{c}{2}$};;
\draw[pattern=north west lines,pattern color=red][preaction={fill=blue!20}] (3.5,1.9) -- (4.5,1.9) -- (4.5,1.7) -- (3.5,1.7) -- cycle node at (4.8,1.8) {$A_u^3$};;
\draw[pattern=grid,pattern color=blue][preaction={fill=red!50}]   (3.5,1.4) -- (4.5,1.4) -- (4.5,1.2) -- (3.5,1.2) -- cycle node at (4.8,1.2) {$A_u^4$};;
\draw[fill=blue,blue]   (1.5,1.9) -- (2.5,1.9) -- (2.5,1.7) -- (1.5,1.7) -- cycle node at (2.8,1.8) {$A_u^1$};;
\draw[pattern=north east lines,pattern color=violet][preaction={fill=green!30}] (1.5,1.4) -- (2.5,1.4) -- (2.5,1.2) -- (1.5,1.2) -- cycle node at (2.8,1.2) {$A_u^2$};;

\draw[fill=blue,blue]  (3.5,0) -- (4.5,0) -- (4.5,-0.3) -- (3.5,-0.3) -- cycle;
\draw[fill=blue,blue]  (0,0) -- (1,0) -- (1,-0.3) -- (0,-0.3) -- cycle;
\draw[fill=blue,blue]  (-0.5,0) -- (-1,0) -- (-1,-0.3) -- (-0.5,-0.3) -- cycle;


\draw[pattern=north east lines,pattern color=violet][preaction={fill=green!30}] (3.5,-0.6) -- (4.5,-0.60) -- (4.5,-0.3) -- (3.5,-0.3) -- cycle;
\draw[pattern=north east lines,pattern color=violet][preaction={fill=green!30}]  (0,-0.6) -- (1,-0.6) -- (1,-0.3) -- (0,-0.3) -- cycle;
\draw[pattern=north east lines,pattern color=violet][preaction={fill=green!30}]  (3,0) -- (3.5,0) -- (3.5,-0.3) -- (3,-0.3) -- cycle;

\draw[pattern=north west lines,pattern color=red][preaction={fill=blue!20}] (-3.5,0) -- (-4.5,0) -- (-4.5,-0.3) -- (-3.5,-0.3) -- cycle;
\draw[pattern=north west lines,pattern color=red][preaction={fill=blue!20}] (0,-0.60) -- (-1,-0.60) -- (-1,-0.3) -- (0,-0.3) -- cycle;
\draw[pattern=north west lines,pattern color=red][preaction={fill=blue!20}] (0.5,-0.6) -- (1,-0.6) -- (1,-0.3) -- (0.5,-0.3) -- cycle;

\draw[pattern=grid,pattern color=blue][preaction={fill=red!50}](-3.5,-0.6) -- (-4.5,-0.6) -- (-4.5,-0.3) -- (-3.5,-0.3) -- cycle;
\draw[pattern=grid,pattern color=blue][preaction={fill=red!50}] (0,-0.6) -- (-1,-0.6) -- (-1,-0.9) -- (0,-0.9) -- cycle;
\draw[pattern=grid,pattern color=blue][preaction={fill=red!50}]  (-3,-0.3) -- (-3.5,-0.3) -- (-3.5,-0.6) -- (-3,-0.6) -- cycle;
%\draw [gray,<->] (-3.5,-1.3) -- (-4.5,-1.3);
%\draw [gray,<->] (3.5,-1.3) -- (4.5,-1.3);

\draw [gray,<->] (0,-1.3) -- (0.5,-1.3);
\draw [gray,<->] (0,-1.3) -- (-.5,-1.3);
\draw [black,<->] (-3.50,-1.3) -- (-3,-1.3);
\draw [black,<->] (3.50,-1.3) -- (3,-1.3);




%
%
\draw [gray,<->] (-5,0) -- (5,0);
%\draw [gray,dashed] (4.5,0) -- (4.5,-1.4);
\draw [gray,dashed] (0.5,0) -- (0.5,-1.4);
\draw [gray,dashed] (0,0) -- (0,-1.4);
\draw [gray,dashed] (-0.5,0) -- (-0.5,-1.4);
\draw [gray,dashed] (-3,0) -- (-3,-1.4);
\draw [gray,dashed] (-3.5,0) -- (-3.5,-1.4);
\draw [gray,dashed] (3.5,0) -- (3.5,-1.4);

%\draw [gray,dashed] (-4.5,0) -- (-4.5,-1.4);

\draw [gray,dashed] (3,0) -- (3,-1.4);
\draw node[anchor=south] at (3.5,0) {$b$};
\draw node[anchor=south] at (4.5,0) {$a$};
\draw node[anchor=south] at (-3.5,0) {$-b$};
\draw node[anchor=south] at (-4.5,0) {$-a$};
\draw node[anchor=south] at (-1,0) {$-c$};

\draw node[anchor=south] at (1,0) {$c$};

%\draw [blue, line width=1pt,<->] (3.5,-0.5) -- (4.5,-0.5);
%\draw [blue, line width=1pt,<->] (0,-0.5) -- (0.5,-0.5);
%
%\draw [violet, line width=1pt,<->] (3.5,-0.8) -- (4.5,-0.8);
%\draw [violet, line width=1pt,<->] (-3.5,-0.8) -- (-3,-0.8);
%
%\draw [red, line width=1pt,<->] (-3.5,-1.1) -- (-4.5,-1.1);
%\draw [red, line width=1pt,<->] (0,-1.1) -- (-0.5,-1.1);
%
%
%\draw [green, line width=1pt,<->] (3.5,-1.4) -- (4,-1.4);
%\draw [green, line width=1pt,<->] (-3.5,-1.4) -- (-4.5,-1.4);
\filldraw [black] (0,0) circle (2pt)node[anchor=south] at (0,0) {$u$};
\end{tikzpicture}
\caption{The representation of different intervals corresponding to each random variable as described in Corollary \ref{cor:extra}}
\end{figure}


\begin{enumerate}
\item $d(u,x) \in [b\frac{\log n}{n},a\frac{\log n}{n}] \cup [0,c\frac{\log n}{n}]  \cup [\frac{-c\log n}{n},\frac{-c/2\log n}{n}]\} \text{ for } i=1$
\item $d(u,x) \in [b\frac{\log n}{n},a\frac{\log n}{n}] \cup [0,c\frac{\log n}{n}]  \cup [\frac{b-c/2\log n}{n},\frac{(a-c)\log n}{n}]\} \text{  for  } i=2$
\item $d(u,x) \in [-a\frac{\log n}{n},-b\frac{\log n}{n}] \cup [-c\frac{\log n}{n},0]  \cup  [\frac{c/2\log n}{n},\frac{c\log n}{n}]\} \text{  for  } i=3$
\item $d(u,x) \in [-a\frac{\log n}{n},-b\frac{\log n}{n}] \cup [-c\frac{\log n}{n},0]  \cup [\frac{(c-a)\log n}{n},\frac{(c/2-b)\log n}{n}]\} \text{  for  } i=4$
\end{enumerate}

\begin{align*}
\Pr(A_u^i=1)&=
\begin{cases}
\Big(1-(c+a-b+(a-b-c/2))\frac{\log n}{2\pi n}\Big)^{n} \text{ when }a-c<b \text{ and } b-c/2 > c\\
\Big(1-(b-c)\frac{\log n}{2\pi n}\Big)^{ n} \text{ when }a-c<b \text{ and } b-c/2 < c\\
\Big(1-(a)\frac{\log n}{2\pi n}\Big)^{n} \text{ when }a-c\ge b \text{ and } b-c/2 < c\\
\Big(1-(c+a-b+c/2)\frac{\log n}{2\pi n}\Big)^{n} \text{ when }a-c \ge b \text{ and } b-c/2 \ge c\\
\end{cases}
\end{align*}
%Notice that $\Pr(A^i_u=1)=\Big(1-(c+a-b+\min\{c/2,a-b-c/2\})\frac{\log n}{n}\Big)^{n}$ when $a-c<b$ and $b-c/2 > b$ and therefore $\sum_{i,u} \avg A^i_u=2n^{1-1.5(\alpha-\beta)}+2\max\{n^{1-1.5(\alpha-\beta)},n^{1-\alpha}\}$ and therefore for $\alpha-\beta \ge 0.67$ and $\alpha \ge 1$, there exists nodes fulfilling all the above conditions for every node $u$ almost surely. This analysis can be done for the other regions as well and hence for every node $u$, there exists nodes in $A_1^u,A_2^u,A_3^u$ and $A_4^u$ for every node $u$ by a simple union bound. 
%Observe that the constraint $\alpha<3\beta$ results in the regions $[0,\frac{\alpha-\beta}{2}\frac{\log n}{n}],[-\beta\frac{\log n}{n},\frac{-\alpha-\beta}{2}\frac{\log n}{n}],[\frac{-\alpha+\beta}{2}\frac{\log n}{n},0]$ and $[\beta\frac{\log n}{n},\frac{\alpha+\beta}{2}\frac{\log n}{n}]$ to have no overlap and therefore they are disjoint regions. 
Notice that $A_u^1$ and $A_u^2$ being zero implies that either there is a node in $\{x \mid d(u,x) \in [b\frac{\log n}{n},a\frac{\log n}{n}]\cup [0,c\frac{\log n}{n}] \}$ or there exists nodes $(v_1,v_2)$ in $\{x \mid d(u,x) \in [\frac{-c\log n}{n},\frac{-c/2\log n}{n}]\}$ and $\{x \mid d(u,x) \in  [\frac{b-c/2\log n}{n},\frac{(a-c)\log n}{n}]\}$. In the second case, $u$ is connected to $v_1$ and $v_1$ is connected to $v_2$. Therefore $u$ has nodes on left and right and $u$ is connected to both of them although not directly. Similarly $A_u^3$ and $A_u^4$ being zero implies that there exist nodes in $\{x \mid d(u,x) \in  [-a\frac{\log n}{n},-b\frac{\log n}{n}]\cup [-c\frac{\log n}{n},0]\}$ or again $u$ will have nodes on left and right and will be connected to them. So , when all the $4$ events happen together, the only exceptional case is when there are nodes in $\{x \mid d(u,x) \in [b\frac{\log n}{n},a\frac{\log n}{n}]\cup [0,c\frac{\log n}{n}] \}$ and $\{x \mid d(u,x) \in  [-a\frac{\log n}{n},b\frac{\log n}{n}]\cup [-c\frac{\log n}{n},0] \}$. But in that case $u$ has direct neighbors on both its left and right. So, we can conclude that for every node $u$, there exists a node $v$ such that $d(u,v) \in[0,\frac{a\log n}{n}]$ and a node $w$ such that $d(u,w) \in[\frac{-a\log n}{n},0]$ such that $u$ is connected to both $v$ and $w$. This implies that every node $u$ has neighbors on both its left and right  and therefore every node is part of a cycle that covers $[0,2\pi]$. % {\color{red} The rest of the proof goes in the same way as Lemma \ref{lem:conninf} and hence we are done.}
\end{proof}


\begin{lemma}\label{lem:rgglower}
A random geometric graph $G(n,\frac{a \log n}{n})$ will have $\omega(1)$ disconnected components for $a <2\pi.$
\end{lemma}
\begin{proof}
Define an indicator random variable $A_u$ for a node $u$ which is $1$ if it does not have a neighbor on its left. We must have that 
\begin{align*}
\Pr(A_u)=\Big(1-\frac{a \log n}{2\pi n}\Big)^{n-1}.
\end{align*}
Therefore we must have that $\sum_u \avg A_u =n^{1-a}=\Omega(1)$ if $a<1$. This statement also holds true with high probability. To show this we need to prove that the variance of $\sum_u \avg A_u$ is bounded. We have that 
\begin{align*}
{\rm Var}(A) <\avg[A]+\sum_{u \neq v} {\rm Cov}(A_u,A_v)=\avg[A]+\sum_{u \neq v} \Pr(A_u=1 \cap A_v=1)-\Pr(A_u=1)\Pr(A_v=1)
\end{align*}
Now, consider the scenario when the  vertices $u$ and $v$ are at a distance more than $\frac{2a \log n}{n}$ apart (happens with probability at least $1-\frac{4a\log n}{2\pi n})$. Then the region in $[0,2\pi]$ that is within distance $\frac{a\log n}{n}$ from both of the vertices is empty and therefore $\Pr(A_u=1 \cap A_v=1) =  \Pr(A_u=1)\Pr(A_v=1) = (\Pr(A_u=1))^2$.  When the vertices  are within distance $\frac{2a \log n}{n}$ of one another, then
$
\Pr(A_u=1 \cap A_v=1) \le \Pr(A_u=1).
$
Therefore,
\begin{align*}
\Pr(A_u=1 \cap A_v=1) \le (1-\frac{4a\log n}{2\pi n}) (\Pr(A_u=1))^2 + \frac{4a\log n}{2\pi n}\Pr(A_u=1).
\end{align*}
Consequently,
\begin{align*}
\Pr(A_u=1 \cap A_v=1)-\Pr(A_u=1)\Pr(A_v=1) &\le (1-\frac{4a\log n}{2\pi n}) (\Pr(A_u=1))^2 \\+ \frac{4a\log n}{2\pi n}\Pr(A_u=1) -& (\Pr(A_u=1))^2 
\le  \frac{4a\log n}{2\pi n}\Pr(A_u=1).
\end{align*}
Now,
$$
{\rm Var}(A) \le \avg[A] + \binom{n}{2}\frac{4a\log n}{2\pi n}\Pr(A_u=1) \le \avg[A](1+ a/\pi\log n).
$$
By using Chebyshev bound, with probability at least $1-\frac{1}{\log n}$, 
%we can upper bound the probability $\Pr(A_u=1 \cap A_v=1)$ by taking the regions of interest to be the same. Hence
%$$ \Pr(A_i=1 \cap A_j=1) \le \frac{4a \log n}{n}n^{-2(a-b)}+\bigg(1-\frac{4a \log n}{n}\bigg)n^{-4(a-b)}$$ and since $\Pr(A_i=1)\Pr(A_j=1)=n^{-4(a-b)}$, we have that
%$$ {\rm Var}(A) < n^{1-2(a-b)}+\frac{n^{2}}{2}\frac{4a \log n}{n}(n^{-2(a-b)}-n^{-4(a-b)})$$  
%Simplifying, we have that ${\rm Var}(A) < n^{1-2(a-b)}(1+2a\log n)$ which gives us using Chebychev that
$$A >n^{1-a/2\pi}-\sqrt{n^{1-a/2\pi}(1+a/\pi\log n)\log n},$$

Now, observe that if there exists $k$ nodes which do not have a neighbor on one side, then there must exist $k-1$ disconnected components. Hence the number of disconnected components in $G(n,\frac{a \log n}{n})$ is $\omega(1)$.
\end{proof}

%Using Lemma \ref{lem:patches} and Corollary \ref{cor:patches}, we get an improved condition for connectivity as defined by the following Lemma.  
%\begin{lemma}
%A graph $G(V,E)$ generated as a variant of the geometric block model where each node $u$ is connected to nodes $v$ iff $\dist(X_u,X_v)\in \left[0,c\frac{\log n}{n}\right]\cup \left[b\frac{\log n}{n},a\frac{\log n}{n}\right]$ is connected if $a-b+c>1$ or $b-c>0.5$ or\\
%$
%\begin{cases}
%2(a-b)+ c/2 > 1 \text{ when } a-b<c \text{ and }b>3c/2\\
%b-c > 1 \text{ when } a-b<c \text{ and }b\le 3c/2\\
%a > 1 \text{ when } a-b\ge c \text{ and } b\le 3c/2 \\
%(a-b)+ 3c/2  > 1 \text{ when } a-b\ge c \text{ and } b>3c/2\\
%\end{cases}$  
%\end{proof}

%\end{document}


